CGAL Made More Accessible

We introduce bindings that enable the convenient, efficient, and reliable use of software modules of CGAL (Computational Geometry Algorithm Library), which are written in C++, from within code written in Python. There are different tools that facilitate the creation of such bindings. We present a short study that compares three main tools, which leads to the tool of choice. The implementation of algorithms and data structures in computational geometry presents tremendous difficulties, such as obtaining robust software despite the use of (inexact) floating point arithmetic, found in standard hardware, and meticulous handling of all degenerate cases, which typically are in abundance. The code of CGAL extensively uses function and class templates in order to handle these difficulties, which implies that the programmer has to make many choices that are resolved during compile time (of the C++ modules). While bindings take effect at run time (of the Python code), the type of the C++ objects that are bound must be known when the bindings are generated, that is, when they are compiled. The types of the bound objects are instances (instantiated types) of C++ function and class templates. The number of object types that can potentially be bound, in implementation of generic computational-geometry algorithms, is enormous; thus, the generation of the bindings for all these types in advance is practically impossible. Often there are several choices to make, resulting in a prohibitively large number of combinations. We present a system that rapidly generates bindings for desired object types according to user prescriptions, which enables the convenient use of any subset of bound object types concurrently. The introduction of the bindings made them easily accessible to newcomers and practitioners in non-computing fields, as we report in the paper.

==> Makefile <==
LANGUAGE = en_US
DOCUMENTS = cgal_python_bindings.pdf
TEXFILES := $(sort $(wildcard *.tex))

PDFLATEX = pdflatex
PDFLATEXFLAGS = -halt-on-error -file-line-error
BIBTEX = bibtex
BIBTEXFLAGS =

#GRAPHICS_STATIC = $(foreach g, \
#	prototyp.pdf, \
#	pics/$g)

GRAPHICS_STATIC =

GRAPHICS_PDF =

GRAPHICS_PDFTEX = $(foreach g, \
	, \
	graphics/$g.pdf_tex)

BASE_DIR = ./

CMAKE_REL_DIR = cmake/tests/release
CMAKE_DIR = $(BASE_DIR)/$(CMAKE_REL_DIR)
CMAKE_FILES = \
	$(CMAKE_DIR)/epec_fixed_release.cmake \
	$(CMAKE_DIR)/cdlg_release.cmake \
	$(CMAKE_DIR)/aos2_epec_face_extended_release.cmake \
	$(CMAKE_DIR)/bso2_epec_cs_release.cmake \
	$(CMAKE_DIR)/tri3_del_epic_release.cmake \
	$(CMAKE_DIR)/as3_del_compact_parallel_epic_release.cmake \
	$(CMAKE_DIR)/ss_2_cdlg_release.cmake

PYTHON_REL_DIR = src/python_scripts/cgalpy_examples
PYTHON_DIR = $(BASE_DIR)/$(PYTHON_REL_DIR)
PYTHON_FILES = \
	$(PYTHON_DIR)/overlay.py \
	$(PYTHON_DIR)/vertical_decomposition.py \
	$(PYTHON_DIR)/ker_intersection.py \
	$(PYTHON_DIR)/kerd_do_intersect.py \
	$(PYTHON_DIR)/aos2_fex.py \
	$(PYTHON_DIR)/Boolean_set_operations_2/circle_segment.py \
	$(PYTHON_DIR)/Boolean_set_operations_2/circle_segment.py \
	$(PYTHON_DIR)/approx_inset.py \
	$(PYTHON_DIR)/tri3_del.py \
	$(PYTHON_DIR)/as3_del_compact_epic.py \
	$(PYTHON_DIR)/kd_tree.py


cgal_python_bindings.pdf: $(PYTHON_FILES) \
	header.tex \
	abrev.bib \
	cgal_python_bindings.tex \
	abstract.tex \
	concepts.tex \
	introduction.tex \
	comparison.tex \
	generation.tex \
	modules.tex \
	code.tex \
	cgal.bib cgal_python_bindings.bib
#	$(GRAPHICS_STATIC) $(GRAPHICS_PDF) $(GRAPHICS_PDFTEX)

.DEFAULT_GOAL = all
.PHONY: all todo spellcheck clean

all: $(DOCUMENTS)

todo:
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		grep -hnT TODO $$texfile || true; \
		grep -hnTo '\\\(todo\|missingfigure\)\(\[.*\]\)\?{.*}' $$texfile | detex || true; \
	done

spellcheck:
	for texfile in $(TEXFILES); do \
		aspell --lang=$(LANGUAGE) check $$texfile; \
	done

$(DOCUMENTS): %.pdf: %.tex
	$(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}
	if grep -e '\citation' -e '\bibdata' -e '\bibstyle' *.aux; then \
		$(BIBTEX) $(BIBTEXFLAGS) $* && $(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}; \
	fi
	$(PDFLATEX) $(PDFLATEXFLAGS) -recorder \\input{$<}
	grep '^OUTPUT ' $*.fls \
		| sed -e 's/^OUTPUT //' \
		| grep -vx $@ \
		| xargs rm
	rm $*.fls
	rm -f $*.bbl $*.blg

%.ps: %.pdf
	pdf2ps -dLanguageLevel=3 $< $@

$(GRAPHICS_PDF): %.pdf: %.svg
	inkscape --without-gui --export-pdf=$*.pdf $*.svg

$(GRAPHICS_PDFTEX): %.pdf_tex: %.svg
	inkscape --without-gui --export-latex --export-pdf=$*.pdf $*.svg

clean:
	rm -f $(DOCUMENTS)
	rm -f *.aux *.bbl *.blg *.log *.out
#	rm -f $(GRAPHICS_PDF)
#	rm -f $(GRAPHICS_PDFTEX)
#	rm -f $(GRAPHICS_PDFTEX:.pdf_tex=.pdf)


==> submission/Makefile <==
LANGUAGE = en_US
DOCUMENTS = cgal_python_bindings.pdf
TEXFILES := $(sort $(wildcard *.tex))

PDFLATEX = pdflatex
PDFLATEXFLAGS = -halt-on-error -file-line-error
BIBTEX = bibtex
BIBTEXFLAGS =

#GRAPHICS_STATIC = $(foreach g, \
#	prototyp.pdf, \
#	pics/$g)

GRAPHICS_STATIC =

GRAPHICS_PDF =

GRAPHICS_PDFTEX = $(foreach g, \
	, \
	graphics/$g.pdf_tex)

BASE_DIR = ./

CMAKE_REL_DIR = cmake/tests/release
CMAKE_DIR = $(BASE_DIR)/$(CMAKE_REL_DIR)
CMAKE_FILES = \
	$(CMAKE_DIR)/epec_fixed_release.cmake \
	$(CMAKE_DIR)/cdlg_release.cmake \
	$(CMAKE_DIR)/aos2_epec_face_extended_release.cmake \
	$(CMAKE_DIR)/bso2_epec_cs_release.cmake \
	$(CMAKE_DIR)/tri3_del_epic_release.cmake \
	$(CMAKE_DIR)/as3_del_compact_parallel_epic_release.cmake \
	$(CMAKE_DIR)/ss_2_cdlg_release.cmake

PYTHON_REL_DIR = src/python_scripts/cgalpy_examples
PYTHON_DIR = $(BASE_DIR)/$(PYTHON_REL_DIR)
PYTHON_FILES = \
	$(PYTHON_DIR)/overlay.py \
	$(PYTHON_DIR)/vertical_decomposition.py \
	$(PYTHON_DIR)/ker_intersection.py \
	$(PYTHON_DIR)/kerd_do_intersect.py \
	$(PYTHON_DIR)/aos2_fex.py \
	$(PYTHON_DIR)/Boolean_set_operations_2/circle_segment.py \
	$(PYTHON_DIR)/approx_inset.py \
	$(PYTHON_DIR)/tri3_del.py \
	$(PYTHON_DIR)/as3_del_compact_epic.py \
	$(PYTHON_DIR)/kd_tree.py


cgal_python_bindings.pdf: $(PYTHON_FILES) \
	../../header.tex \
	../../abrev.bib \
	cgal_python_bindings.tex \
	abstract.tex \
	concepts.tex \
	introduction.tex \
	comparison.tex \
	generation.tex \
	modules.tex \
	code.tex \
	extenders.tex \
	../../cgal.bib ../cgal_python_bindings.bib
#	$(GRAPHICS_STATIC) $(GRAPHICS_PDF) $(GRAPHICS_PDFTEX)

.DEFAULT_GOAL = all
.PHONY: all todo spellcheck clean

all: $(DOCUMENTS)

todo:
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		grep -hnT TODO $$texfile || true; \
		grep -hnTo '\\\(todo\|missingfigure\)\(\[.*\]\)\?{.*}' $$texfile | detex || true; \
	done

spellcheck:
	for texfile in $(TEXFILES); do \
		aspell --lang=$(LANGUAGE) check $$texfile; \
	done

$(DOCUMENTS): %.pdf: %.tex
	$(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}
	if grep -e '\citation' -e '\bibdata' -e '\bibstyle' *.aux; then \
		$(BIBTEX) $(BIBTEXFLAGS) $* && $(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}; \
	fi
	$(PDFLATEX) $(PDFLATEXFLAGS) -recorder \\input{$<}
	grep '^OUTPUT ' $*.fls \
		| sed -e 's/^OUTPUT //' \
		| grep -vx $@ \
		| xargs rm
	rm $*.fls
	rm -f $*.bbl $*.blg

%.ps: %.pdf
	pdf2ps -dLanguageLevel=3 $< $@

$(GRAPHICS_PDF): %.pdf: %.svg
	inkscape --without-gui --export-pdf=$*.pdf $*.svg

$(GRAPHICS_PDFTEX): %.pdf_tex: %.svg
	inkscape --without-gui --export-latex --export-pdf=$*.pdf $*.svg

clean:
	rm -f $(DOCUMENTS)
	rm -f *.aux *.bbl *.blg *.log *.out
#	rm -f $(GRAPHICS_PDF)
#	rm -f $(GRAPHICS_PDFTEX)
#	rm -f $(GRAPHICS_PDFTEX:.pdf_tex=.pdf)


==> submission/code.tex <==
% =============================================================================
\section{Binding code}
\label{sec:code}
% =============================================================================
Nanobind allows users to expose C++ classes and functions to Python using nothing more than a C++ compiler. It exploits metaprogramming techniques to implement a rich set of features and high-level user-friendly interface. Nanobind extracts as much as information as possible from the source code to be wrapped. This approach is referred to as \emph{user guided wrapping}. Additional information that cannot be automatically deduced is explicitly supplied by the user. The interface specification is written in the same full-featured C++ language as the code being exposed, which has the potential of generating efficient binding. In this section we describe some of the techniques we use to ensure that.

% -----------------------------------------------------------------------------
\subsection{Return value policy}
\label{sec:code:rvp}
% -----------------------------------------------------------------------------
Python and C++ use fundamentally different ways of managing the memory and lifetime of objects. This can lead to issues when creating bindings for functions that return a non-trivial type. Just by looking at the type, it is unclear whether Python should take charge of the returned value and eventually free its resources, or whether this is handled by the C++ code. When writing code in C++, it is usually considered a good practice to use smart pointers, which exactly describe ownership semantics. Still, even good C++ interfaces use raw references and pointers sometimes. In some cases, in order to assure proper memory management of a return value from a function, explicitly specifying a return value policy is needed. The policy may depend on whether the returned object is a newly created object, a reference to some already existing (internal) object, or a \cppLstinline{const} reference to some existing object. Additionally, in some cases we need to tie the lifetime of the result to the lifetime of the arguments, or the other way around.

For some functions of kernel objects the kind of return value depends on the kernel type; thus, the return value policy needs to be set accordingly. For example, when \cppLstinline{Exact\_predicates\_exact\_constructions\_kernel} is the kernel type, the return type of some functions that return a coordinate or a coefficient is a \cppLstinline{const} reference, while when the kernel type is \cppLstinline{Exact\_predicates\_inexact\_constructions\_kernel} the same functions return an object by value. This is why for these functions a \myLstinline{Kernel_return_value_policy} type is being passed as the return value policy. The type is defined differently based on the kernel being exposed.

%% All functions and classes related to some package were exposed inside
%% a \myLstinline{export_[package]()} function. All such calls are
%% happening in \myLstinline{export_module.cpp}. We wrap each call with a
%% local (C++) scope and call the \myLstinline{SET_SCOPE(module_name)}
%% macro, which causes every exposed function/class inside this local
%% scope to be exposed inside the \myLstinline{module_name} submodule of
%% the CGALPY module. This prevents name clashes of classes with the same
%% name in different packages.

%% % -----------------------------------------------------------------------------
%% \subsection{Avoiding Code Duplication}
%% \label{sec:code:templates}
%% % -----------------------------------------------------------------------------
%% Some types have the exact same nested types and member functions
%% exposed, e.g., \cppLstinline{Triangulation\_2} and
%% \cppLstinline{Delaunay\_triangulation\_2} class templates each have
%% the method \cppLstinline{dimension()} exposed as the Python attribute
%% \pyLstinline{dimension}. In these cases we use a function template to
%% avoid code duplication. Following the example above, we have the
%% function \cppLstinline{export\_triangulation\_2<Triangulation>()},
%% where the template parameter \cppLstinline{Triangulation} is
%% substituted with one of the two-dimensional triangulation types
%% supported; see Table~\ref{tab:tri2:names}. This function template
%% accepts as its single parameter the binding class object, which is
%% constructed separately.

%% \begin{lstlisting}[style=cppNumberedStyle]
%% typedef CGAL::Triangulation_2<Kernel>              Triangulation_2;
%% typedef CGAL::Delaunay_triangulation_2<Kernel>     Delaunay_triangulation_2;

%% auto c0 = py::class_<Triangulation_2>("Triangulation_2");
%% auto c1 = py::class_<Delaunay_triangulation_2,
%%                      py::bases<Triangulation_2>>("Delaunay_triangulation_2");

%% export_triangulation_2<Triangulation_2>(c0);
%% export_triangulation_2<Delaunay_triangulation_2>(c1);
%% \end{lstlisting}

% -----------------------------------------------------------------------------
\subsection{Intersection Detection}
\label{sec:code:intersectionDetection}
% -----------------------------------------------------------------------------
\begin{figure}[!tp]
  \centerline{\begin{tikzpicture}[>=stealth,align=center,every node/.style={font=\sffamily}]
    \tikzstyle{state}=[text centered,node distance=0.5cm,%
      rectangle,rounded corners,fill=white,draw=black,%
      minimum width=1.0cm,minimum height=0.45cm]
    % All state styles
    \tikzstyle{lookup}=[state,bottom color=purple!40]
    \tikzstyle{deduction}=[state,fill=orange!40]
    \tikzstyle{reduction}=[state,fill=yellow!40]
    \tikzstyle{selection}=[state,fill=green!40]
    % All states
    \node (lookup)[lookup]{Name Lookup};
    \node (lookupFailure)[below left=0.5 and -1 of lookup]
      {\textcolor{red}{Error: Lookup failure}};
    \node (deduction)[deduction,below right=1 and -1.2 of lookup]
      {Template Argument Deduction};
    \node (deductionFailure)[below left=0.5 and -2.8 of deduction]
      {\textcolor{red}{Error: Deduction failure}};
    \node (reduction)[reduction,below right=1 and -1.2 of deduction] {Reduction};
    \node (reductionFailure)[below left=0.5 and -1.6 of reduction]
      {\textcolor{red}{Error: Substitution failure}};
    \node (selection)[selection,below right=1 and 0.0 of reduction]
      {Final Selection};
    \node (success)[below right=0.5 and -0.7 of selection]{\textcolor{blue}{Best Match}};
    \node (slectionFailure)[below left=0.5 and -1.6 of selection]
      {\textcolor{red}{Error: Ambiguity failure}};
    % Edges
    \draw [thick,->,>=Stealth] (lookup) -- (deduction);
    \draw [thick,->,>=Stealth] (lookup) -- (lookupFailure);
    \draw [thick,->,>=Stealth] (deduction) -- node[anchor=west]{Non-empty candidate Set}(reduction);
    \draw [thick,->,>=Stealth] (deduction) -- (deductionFailure);
    \draw [thick,->,>=Stealth] (reduction) -- node[anchor=west]{Non-empty viable Set} (selection);
    \draw [thick,->,>=Stealth] (reduction) -- (reductionFailure);
    \draw [thick,->,>=Stealth] (selection) -- (success);
    \draw [thick,->,>=Stealth] (selection) -- (slectionFailure);
  \end{tikzpicture}}
  \caption{Overload resolution steps}
  \label{fig:ors}
\end{figure}

The function template \cppLstinline{CGAL::do_intersect(const T1& o1, const T2& o2)} determines whether two geometric objects intersect. The function is overloaded with several implementations that handle different combinations of types of arguments provided by the \iiDandiiiDGeometryKernelPackage{} package (see Section~\ref{ssec:modules:kernel}). However, not every combination of two types is implemented in this package. For example, the intersection of a line segment and a circle in the general case is a point with algebraic coordinates, and thus not supported by the package.\footnote{For a complete list of valid combinations of \cppLstinline{do_intersect()} argument types refer to the reference manual at   \url{https://doc.cgal.org/latest/Kernel_23/group__do__intersect__linear__grp.html}.} We use \emph{substitution failure is not an error} (SFINAE) to generate bindings for all supported combinations while avoiding getting compilation errors for unsupported combinations. SFINAE refers to a situation in C++ where an invalid substitution of template parameters should not be treated as an error. In particular, it may occur during a process called \emph{overload resolution}. In order to compile a function call, the compiler creates a set of candidate functions the names of which match the call and that can be accessed by the caller. Then, it reduces the candidate set to a set of viable functions that includes all function instances the parameters of which match the call arguments. Finally, the compiler selects the best match among the viable functions according to the C++ standard;\footnote{For the full specification of the C++ standard see \url{https://isocpp.org/std/the-standard}.} a flowchart that describes the process is shown in Figure~\ref{fig:ors}. When the substitution of an explicitly specified or deduced type for the template parameter fails, the specialization is discarded from the overload set instead of causing a compilation error.\footnote{For more information on SFINAE see, e.g., \url{https://en.cppreference.com/w/cpp/language/sfinae}.}

Our entry point is the function \cppLstinline{export_intersections_2(py::module_& m)}; see Line~8 in Listing~\ref{lst:exportIntersection}. It accepts a wrapper for Python extension modules, which is used to wrap the \cppLstinline{CGAL::do_intersect()} functions (Line 7 in Listing~\ref{lst:do_intersect}). It also serves as the entry point for the generation of bindings for the function \cppLstinline{CGAL::intersection(const T1& o1, const T2& o2)}; see Section~\ref{sec:code:intersectionComputation}. Let $\calT_2$ and $\calT_3$ denote the complete sets of types of two-dimensional and three-dimensional objects, respectively, supported by the \iiDandiiiDGeometryKernelPackage{} package; see Listing~\ref{lst:exportIntersection} Lines~9--12. Our goal is the automatic instantiation of the class template \cppLstinline{Wrapper} (Listing~\ref{lst:exportIntersection} Line 1) for every pair (\cppLstinline{T1}, \cppLstinline{T2}) in the Cartesian products $\calT_2 \times \calT_2$ and $\calT_3 \times \calT_3$, where the template parameter pack \cppLstinline{... Types} is substituted with the pair \cppLstinline{T1}, \cppLstinline{T2}. In particular, we seek for the evaluation of the expression \cppLstinline{Wrapper<T1, T2>::operator()(m)} for each instance, which in turn, leads to the evaluation of the expression \cppLstinline{bind_do_intersect<T1, T2>(m, true)} for every such pair. The expansion of the constant expression in Line~13 of Listing~\ref{lst:exportIntersection} as part of the compilation process results in the evaluation of the expression \cppLstinline{Wrapper<T1, T2>::operator()(m)} for each (\cppLstinline{T1}, \cppLstinline{T2}) $\in \calT_2 \times \calT_2$. Similarly, the expansion of the constant expression in Line~14 of Listing~\ref{lst:exportIntersection} results in the evaluation of the expression \cppLstinline{Wrapper<T1, T2>::operator()(m)} for each (\cppLstinline{T1}, \cppLstinline{T2}) $\in \calT_3 \times \calT_3$.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:exportIntersection},%
                     caption={Entry points for the code that automatically generates
                     binding for \cppLstinline{CGAL::do_intersect()} and
                     \cppLstinline{CGAL::intersection()} with arguments
                     that represent planar geometric objects.}]
template <typename Arg, typename ... Types> struct Wrapper {
  void operator()(Arg& arg) {
    bind_do_intersect<Types...>(arg, true);
    bind_intersection<Types...>(arg, true);
  }
};

void export_intersections_2(py::module_& m) {
  CGALPY::Type_list<Iso_rectangle_2, Line_2, Ray_2, Segment_2, Triangle_2,
                    Point_2, Circle_2> type_list_2;
  CGALPY::Type_list<Iso_cuboid_3, Line_3, Ray_3, Segment_3, Tetrahedron_3,
                    Triangle_3, Point_3, Sphere_3> type_list_3;
  cartesian_product<Wrapper>(m, type_list_2, type_list_2);
  cartesian_product<Wrapper>(m, type_list_3, type_list_3);
}
  \end{lstlisting}
\end{lstfloat}

The function template \cppLstinline{cartesian_product} (see Listing~\ref{lst:cartesianProduct} Line~17) can be used to evaluate expressions for each member of the Cartesian product of a given sequence of sets of types.  The code in Listing~\ref{lst:cartesianProduct} was presented to us, so we merely provide the code. When the template function is instantiated the \cppLstinline{Wrap} template parameter must be substituted with a class template that has an \cppLstinline{operator()} member function. The template class that substitutes the \cppLstinline{Wrap} template parameter is instantiated for every member of the Cartesian product of the sets of types that are used to define the types of the \cppLstinline{type_lists} argument pack. Observe that the type of each object in this pack is an instance of the class template \cppLstinline{Type_list}, which in turn is defined by substituting a template parameter pack with a sequence of types. The \cppLstinline{arg} argument is propagated all the way and passed to the \cppLstinline{operator()} member function of the wrapper instantiated object. Finally, the expression \cppLstinline{Wrap<T1, T2>::operator()(arg)} is evaluated for every member of the Cartesian product.
The function \cppLstinline{cartesian_product} is implemented with the help of the (compile-time) recursive function template \cppLstinline{cartesian_product_recursive()}, which exploits a unary right fold expression; see Listing~\ref{lst:cartesianProduct} Line 13.\footnote{For more information about fold expressions see \url{https://en.cppreference.com/w/cpp/language/fold}.} Let $\mathrm{E}$ denote an expression that contains a variadic template pack $\mathrm{\calT}$. Consider a block of code that contains a unary right fold expression $(\mathrm{E}\,op\,...)$, and assume that the template pack $\mathrm{\calT}$ is substituted with the sequence of types $\mathrm{T}_1,\mathrm{T}_2,\ldots,\mathrm{T}_n$, when the code block is instantiated. The unary right fold expression $(\mathrm{E}\,op\,...)$ expands to $(\mathrm{E}_1\,op\,(\ldots\,op\,(\mathrm{E}_{n-1}\,op\,\mathrm{E}_n)))$, where $\mathrm{E}_i$ is the expression $\mathrm{E}$ with the template pack $\mathrm{\calT}$ substituted with $\mathrm{T}_i$. In our case (lines 13-14 in the listing) (i) $op$ is the (binary) comma operator,\footnote{For more information about the comma operator see \url{https://en.cppreference.com/w/cpp/language/operator_other\#Built-in_function_call_operator}.} (ii) $\mathrm{E}$ is the recursive call to \cppLstinline{cartesian_product_recursive()}, and (iii) the variadic template pack is \cppLstinline{... Types}. Let \cppLstinline{type_lists_1}, \cppLstinline{type_lists_2},\ldots,\cppLstinline{type_lists_m} denote the sequence of objects that comprise the \cppLstinline{type_lists} argument pack. In all evaluations of the recursive expression at level $i$ of the recursion tree, that represents the iterated recurrence, the template pack \cppLstinline{... Types} is substituted with the sequence of types that are used to define the type of the \cppLstinline{type_lists_i}.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:cartesianProduct},%
                     caption={Automatic expansion of expressions with types that
                     are members of the Cartesian product of sets of types.}]
template <typename... Types> class Type_list {};

template <typename... Types> class Call_args {};

template <template <typename ...> class Wrapper, typename Arg, typename... Types>
void cartesian_product_recursive(Arg& arg, Call_args<Types...>)
{ Wrapper<Arg, Types...>()(arg); }

template <template <typename ...> class Wrapper, typename Arg,
          typename... CallTypes, typename... Types, typename ... TypeLists>
void cartesian_product_recursive(Arg& arg, Call_args<CallTypes...>,
                                 Type_list<Types...>, TypeLists... type_lists) {
  (cartesian_product_recursive<Wrapper>(arg, Call_args<CallTypes..., Types>(),
                                        type_lists...), ...);
}

template <template <typename ...> class Wrapper, typename Arg, typename... TypeLists>
void cartesian_product(Arg& arg, TypeLists... type_lists) {
  cartesian_product_recursive<Wrapper>(arg, Call_args<>(), type_lists...);
}
  \end{lstlisting}
\end{lstfloat}

Consider two types \cppLstinline{Type1} and \cppLstinline{Type2}, and assume that the \cppLstinline{CGAL::do_intersect(const Type1& o1, const Type2& o2)} overloaded version is not implemented but all other three combinations in the Cartesian product of \{\cppLstinline{Type1}, \cppLstinline{Type2}\}$\times$\{\cppLstinline{Type1}, \cppLstinline{Type2}\} are, and refer to Listing~\ref{lst:do_intersect}. The \cppLstinline{bind_do_intersect()} function template is overloaded with two implementations (Line~5 and~7). As a consequence, assuming that the code compiles, one overload of \cppLstinline{bind_do_intersect()} is selected for every member of the Cartesian product of \{\cppLstinline{Type1}, \cppLstinline{Type2}\}$\times$\{\cppLstinline{Type1}, \cppLstinline{Type2}\}. The primary implementation of \cppLstinline{bind_do_intersect()} (Line~1) uses \emph{variadic arguments} and serves as a fall-through when the evaluation of the second implementation fails during the resolution process.\footnote{For more information on \emph{variadic arguments} see \url{https://en.cppreference.com/w/cpp/language/variadic_arguments}.} The type of the second parameter of the second implementation is defined as the return type of \cppLstinline{CGAL::do_intersect<Kernel>(T1(), T2())}. When \cppLstinline{T1} and \cppLstinline{T2} are substituted with \cppLstinline{Type1} and \cppLstinline{Type2}, respectively, the evaluation fails, and the blank implementation is selected, as this is the only candidate left. In all other three cases the evaluation succeeds and the second implementation is selected, as functions that accept variadic arguments have a lower rank for the purpose of overload resolution.
% The return type of \cppLstinline{CGAL::do_intersect<Kernel>(T1(), T2())} is resolved at compile time.
Observe that in the call to \cppLstinline{bind_do_intersect()} (Line~2) we pass a \cppLstinline{bool} argument of value \cppLstinline{true}. This value can be \cppLstinline{false} just as well, but its type, that is \cppLstinline{bool}, must match the return type of \cppLstinline{CGAL::do_intersect<Kernel>(T1(), T2())} when defined. The result is not only compact code that is easy to maintain, but also code that supports bindings for every potential \cppLstinline{do_intersect()} overload that might be implemented in the future.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:do_intersect},%
                     caption={Automatic generation of binding  for \cppLstinline{CGAL::do_intersect()} exploiting SFINAE.}]
template <typename, typename> void bind_do_intersect(py::module_&, ...) {}

template <typename T1, typename T2>
void bind_do_intersect(py::module_& m,
                       decltype(CGAL::do_intersect<Kernel>(T1(), T2()))) {
  using Do_intersect = bool(*)(const T1&, const T2&);
  m.def("do_intersect", static_cast<Do_intersect>(&CGAL::do_intersect<Kernel>));
}
  \end{lstlisting}
\end{lstfloat}

% function \cppLstinline{bind_do_intersect()} calls
%\cppLstinline{bind_do_intersect_1T<T1>()} twice; in the first call
%\cppLstinline{T1} is substituted with \cppLstinline{Type1} (Line~15)
%and in the second call \cppLstinline{T1} it is substituted with
%\cppLstinline{Type2} (Line~16).  The function template
%\cppLstinline{bind_do_intersect_1T()} calls a third function, called
%\cppLstinline{bind_do_intersect_pair{}, twice; first it calls
%cppLstinline{bind_do_intersect_pair<T1, Type1>(true)} (Line~10); then,
% it calls \cppLstinline{bind_do_intersect_pair<T1, Type2>(true)} (Line~11).

% -----------------------------------------------------------------------------
\subsection{Intersection Computation}
\label{sec:code:intersectionComputation}
% -----------------------------------------------------------------------------
The situation presented by the overloaded function template \cppLstinline{CGAL::intersection(const T1& o1, const T2& o2)} that computes the intersection of two geometric objects is a bit more complicated. The various implementations are also provided by the \iiDandiiiDGeometryKernelPackage{} package. Similar to the \cppLstinline{CGAL::do_intersect()} function templates, different implementations handle different combination of types of arguments and not all combinations are supported. The intersection of two geometric objects can be either empty, a single object, or several points. Unlike the \cppLstinline{CGAL::do_intersect()} function templates, the return types of which are all simple \cppLstinline{bool}, the return type of each \cppLstinline{CGAL::intersection()} function template is a polymorphic type that either implicitly converts to \cppLstinline{false} if the intersection is empty or represents the intersection and depends on the types of the input arguments.

The mechanism introduced in the previous section results in the evaluation of the expression \cppLstinline{bind_intersection<T1, T2>(m, true)} for every pair (\cppLstinline{T1}, \cppLstinline{T2}) in the Cartesian products $\calT_2 \times \calT_2 \cup \calT_3 \times \calT_3$; see Listing~\ref{lst:exportIntersection} Line 4. See Line~1 and Line~3 in Listing~\ref{lst:intersection} for the primary and specialized implementations, respectively, of the function template \cppLstinline{bind_intersection()}. Given a combination of two specific types, \cppLstinline{T1} and \cppLstinline{T2}, we still evaluate the return value of the function template \cppLstinline{CGAL::intersection(const T1& o1, const T2& o2)} as a mean to determine whether the function is defined, but we do not try to match this type to a type of an argument. Instead, we introduce an unnamed template parameter with a default value that evaluates to the return type of \cppLstinline{CGAL::intersection(const T1& o1, const T2& o2)}; see Line~4 in the listing. Observe that the outcome of the evaluation is irrelevant. The only thing that matters is whether the evaluation succeeds---it succeeds only if the function template \cppLstinline{CGAL::intersection(const T1& o1, const T2& o2)} is defined. If it is defined, the specialized implementation is selected by the overload-resolution process, and the function \cppLstinline{cgalpy_intersection(const T1& t1, const T2& t2)}, which actually computes the intersection, is exposed; see Listing~\ref{lst:intersectionImpl}.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:intersection},%
                     caption={Automatic generation of binding for \cppLstinline{CGAL::intersection()} exploiting SFINAE}.]
template <typename, typename> void bind_intersection(py::module_& m, ...) {}

template <typename T1, typename T2,
          typename = decltype(CGAL::intersection<Kernel>(T1(), T2()))>
void bind_intersection(py::module_& m, bool)
{ m.def("intersection", &cgalpy_intersection<T1, T2>); }
  \end{lstlisting}
\end{lstfloat}

The exposed Python function that computes the intersection returns \pyLstinline{None} if the intersection is empty; see Line~17 in Listing~\ref{lst:intersectionImpl}. If the intersection consists of a single geometric object, the function returns a single Python object the type of which is the exposed \cgal{} C++ type of the geometric object; see Line~4. Finally, if several points comprise the intersection, the return type is a list of Python objects (see Line~10), where the type of each element in the list is the exposed type of \cppLstinline{Kernel::Point_2}. For more information of functions that return collections of object see Section~\ref{sec:code:output}.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:intersectionImpl},%
                     caption={Implementation of the binding for \cppLstinline{CGAL::intersection()}.}]
class Intersection_visitor : public boost::static_visitor<py::object> {
public:
  template<typename T>
  py::object operator()(T& operand) const { return py::cast(operand); }

  // Handle vector of points
  py::object operator()(std::vector<Point_2>& operand) const {
    py::list lst;
    for (const auto& p : operand) lst.append(p);
    return lst;
  }
};

template <typename T1, typename T2>
py::object cgalpy_intersection(const T1& t1, const T2& t2) {
  auto result = CGAL::intersection<Kernel>(t1, t2);
  if (! result) return py::object();    // no intersection
  return boost::apply_visitor(Intersection_visitor(), *result);
}
  \end{lstlisting}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsection{Minkowski Sum Construction}
\label{sec:code:minkSumComputation}
% -----------------------------------------------------------------------------
The situation presented by the function template \cppLstinline{CGAL::minkowski_sum_2()} that applies the \emph{convex-decomposition approach} (see Section~\ref{ssec:modules:ms2}) is even more complicated. The function template shown in Line~1 of Listing~\ref{lst:minkSumConvexDecomposition} has 10 instances of valid combinations of argument types. There is another set, of the same cardinality, of function templates that also accept a fourth traits parameter. The number of instances of the function template shown in Line~8 is 36, and also here there is another set, of the same cardinality, of function templates that accept an additional traits parameter. Consider the function template shown in Line~1. We need to generate bindings for instances of this function only for valid combinations of \cppLstinline{PolygonType1}, \cppLstinline{PolygonType2}, and \cppLstinline{PolygonConvexDecomposition_2} types. Hereafter and in the code listing we use the respective short names \cppLstinline{PT1}, \cppLstinline{PT2}, and \cppLstinline{PP} instead. A valid combination exists only if \cppLstinline{PP} is a type of a polygon-partition unary function that can be applied to a polygon of type \cppLstinline{PT1} and to a polygon of type \cppLstinline{PT2}. Some supported polygon-partition functions cannot be applied to polygon with holes, hence invalid combinations. In particular, if \cppLstinline{pp} is a polygon-partition function, the calls \cppLstinline{pp(pgn1, it)} and \cppLstinline{pp(pgn2, it)} must be valid, where \cppLstinline{pgn1} and \cppLstinline{pgn2} are input polygons of types \cppLstinline{PT1} and \cppLstinline{PT2}, respectively, and \cppLstinline{it} is an output iterator of a container of the resulting polygons. Dereferencing the iterator must yield a type that can represent a simple polygon. If \cppLstinline{PT1} is identical to \cppLstinline{Polygon_2}, then \cppLstinline{std::list<PT1>::iterator} can serve as an output iterator; otherwise, \cppLstinline{PT1} must represent a polygon with holes, and in this case \cppLstinline{std::list<PT1::Polygon_2>::iterator} can serve as an output iterator; the same holds for \cppLstinline{PT2}. We use SFINAE yet again to make this distinction, \footnote{This usage is similar to the example shown in \url{https://en.wikipedia.org/wiki/Substitution_failure_is_not_an_error\#C++11_simplification}.} and we use SFINAE one more time to generate binding for \cppLstinline{CGAL::minkowski_sum_2()} only for valid combinations of argument types.

\begin{lstfloat}
  \begin{lstlisting}[style=cppframedStyle,basicstyle=\normalsize,%
                     label={lst:minkSumConvexDecomposition},%
                     caption={Signatures of function templates that compute the 2D Minkwoski sum using the convex-decomposition approach.}]
template <typename Kernel, typename Container,
          typename PolygonConvexDecomposition_2>
Polygon_with_holes_2<Kernel, Container>
minkowski_sum_2(const PolygonType1<Kernel, Container>& p,
                const PolygonType2<Kernel, Container>& q,
                const PolygonConvexDecomposition_2& decomp)

template <typename Kernel, typename Container,
          typename PolygonConvexDecompositionP_2,
          typename PolygonConvexDecompositionQ_2>
Polygon_with_holes_2<Kernel, Container>
minkowski_sum_2(const PolygonType1<Kernel, Container>& p,
                const PolygonType2<Kernel, Container>& q,
                const PolygonConvexDecompositionP_2& decomp_p,
                const PolygonConvexDecompositionQ_2& decomp_q)
  \end{lstlisting}
\end{lstfloat}

Our entry point is the function \cppLstinline{void export_minkowski_sum_2()}; see Line~11 in Listing~\ref{lst:minkowskiSumExpansion}. We need to capture valid combinations of three types and valid combinations of four types. Recall that the code in Listing~\ref{lst:do_intersect} captures valid combinations of two types. Following the method presented in the previous section, we introduce two wrapper template classes with \cppLstinline{operator()} members, which call \cppLstinline{bind_mink_sum_one_strategy()} and \cppLstinline{bind_mink_sum_two_strategies()}, respectively; see Line~3 and Line~8 in Listing~\ref{lst:minkowskiSumExpansion}.

\begin{lstfloat}
  \begin{lstlisting}[style=cppframedStyle,basicstyle=\normalsize,%
                     label={lst:minkowskiSumExpansion},%
                     caption={Automatic expansion of expressions that generate
                              bindings for Minkowski-sum computation.}]
template <typename Arg, typename ... Types> struct Wrapper_one_strategy {
  void operator()(Arg& arg)
  { bind_mink_sum_decomp_one_strategy<Types...>(arg, true); }
};

template <typename Arg, typename ... Types> struct Wrapper_two_strategies {
  void operator()(Arg& arg)
  { bind_mink_sum_decomp_two_strategies<Types...>(arg, true); }
};

void export_minkowski_sum_2(py::module_& m) {
  using Pnp = ms2::Polygon_nop_decomposition_2;
  using Pvd = pp2::Polygon_vertical_decomposition_2;
  using Ptd = pp2::Polygon_triangulation_decomposition_2;
  using Ssabd = pp2::Small_side_angle_bisector_decomposition_2;

  CGALPY::Type_list<Polygon_2, Polygon_with_holes_2> polygon_types;
  CGALPY::Type_list<Pnp, Pvd, Ptd, Ssabd> strategy_types;

  CGALPY::cartesian_product<Wrapper_one_strategy>(m, polygon_types, polygon_types,
                                                  strategy_types);
  CGALPY::cartesian_product<Wrapper_two_strategies>(m, polygon_types, polygon_types,
                                                    strategy_types, strategy_types);
}
  \end{lstlisting}
\end{lstfloat}

First, we introduce a class template called \cppLstinline{target}; see Line~3 in Listing~\ref{lst:minkSumResolution}. It is parameterized with a named parameter \cppLstinline{T} and an unnamed parameter that defaults to \cppLstinline{void}. It delegates the \cppLstinline{std::list<T>::iterator} type. We also introduce a specialization (Line 6) that delegates the type \cppLstinline{std::list<T::Polygon_2>::iterator}. The second parameter is substituted with a type provided by a utility template called \cppLstinline{void_t<>} (Line~1). If the type \cppLstinline{T::Polygon_2} is undefined, the evaluation of \cppLstinline{void_t<T::Polygon_2>} fails, and in turn the specialization \cppLstinline{Target<>} is discarded from the overloaded resolution set. Otherwise, \cppLstinline{void_t<T::Polygon_2>} successfully evaluates (to \cppLstinline{void}). In this case the \cppLstinline{Target<>} specialization remains a viable option, and it is selected over the primary implementation, since specializations are ranked higher. Observe that the type delegated by the \cppLstinline{void_t<>} template and the type of the unnamed template parameter of the primary implementation of \cppLstinline{target<>} must match for the ordering to apply. These types are arbitrarily chosen to be \cppLstinline{void}.

We need to capture valid combinations of three types for Minkowski-sum computation using a single convex decomposition strategy and valid combinations of four types for Minkowski-sum computation using two convex decomposition strategies. Recall that the code in the listings of the previous sections captures valid combinations of two types. Following the method presented in the previous sections, we introduce a wrapper template class with an \cppLstinline{operator()} member, which calls \cppLstinline{bind_mink_sum()}; see Lines~10,13 in Listing~\ref{lst:minkSumResolution} for the primary and specialized implementations, respectively. The polygon-partition function returns an output iterator that points to the element, which is next to the last element of the container. Passing an argument, the type of which matches the type of the returned value of the polygon-partition function, to the function \cppLstinline{bind_mink_sum()} is complicated, as this type is not a simple type (e.g., \cppLstinline{bool}) anymore. Instead, we introduce two unnamed template parameters with default values that evaluate to the return types of the polygon-partition function when applied to a polygon of type \cppLstinline{PT1} or \cppLstinline{PT2}, respectively; see Lines~14--15. Observe that the outcome of an evaluation is irrelevant. The only thing that matters is whether the evaluation succeeds---it succeeds only if the matching function is defined.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,
                     label=lst:minkSumResolution,
                     caption={Automatic generation of binding for \cppLstinline{CGAL::minkowski_sum_2}            exploiting SFINAE.}]
template <typename... Ts> using void_t = void;

template <typename T, typename = void> struct target
{ using type = typename std::list<T>::iterator; };

template <typename T>
struct target<T, void_t<typename T::Polygon_2>>
{ using type = typename std::list<typename T::Polygon_2>::iterator; };

template <typename T1, typename T2, typename T3>
void bind_mink_sum(py::module_&, ...) {}

template <typename PT1, typename PT2, typename PP,
          typename = decltype(PP()(PT1(), typename target<PT1>::type())),
          typename = decltype(PP()(PT2(), typename target<PT2>::type()))>
void bind_mink_sum(py::module_& m, bool) {
  m::def<Polygon_with_holes_2(const PT1&, const PT2&, const PP&)>
    ("minkowski_sum_2", &CGAL::minkowski_sum_2<Kernel, Point_2_container, PP>);
}
  \end{lstlisting}
\end{lstfloat}

%% templated with some supported type
%% {T1}. \myLstinline{bind_do_intersect_1T()}, templated with
%% \myLstinline{T1}, calls \myLstinline{bind_do_intersect_2T} templated
%% with \myLstinline{T1} and some supported type \myLstinline{T2}, and a
%% \myLstinline{bool} argument.  The declaration of
%% \myLstinline{bind_do_intersect_2T}, templated with both
%% \myLstinline{T1} and \myLstinline{T2} is only valid when templated
%% with a combination of types for which an overloaded implementation of
%% \myLstinline{CGAL::do_intersect} exists. Otherwise, due to SFINAE, the
%% blank implementation template of \myLstinline{bind_do_intersect_2T}
%% expecting (...) as an argument will be invoked (it would normally not
%% be invoked as variadic parameters have the lowest rank for the purpose
%% of overload resolution).

\noindent%
We exploit SFINAE to generate bindings of other types as described in the following sections.

% -----------------------------------------------------------------------------
\subsection{Arrangement Extension}
\label{sec:code:ae}
% -----------------------------------------------------------------------------
In many applications it is necessary to extend the type that represents certain \cgal{} data structures with some types that represent new properties. In \cgal{} it is more convenient, and thus more common, to extend the types that represent the topological features of the data structures (rather than the types that represent the geometric features), e.g., the DCEL of the arrangement data structure; see Section~\ref{ssec:modules:aos2}. When developing code in pure C++, there is no restriction on the property types used to extend the data structure. However, when the data structure interface is wrapped with Python bindings, the property type must be known when the bindings are compiled. Nevertheless, we support extensions with generic Python objects. If a certain feature must be extended with a certain property, the type of which is defined in the C++ code, it is always possible to use an external property map, where the properties are indexed by a Python object, such as an integer or a string. When generating the bindings the user must set the flag that enables the extension; see Table~\ref{tab:aos}. Attaching an index to and extracting an index from a feature is done via the \cppLstinline{set_data()} and \cppLstinline{data()} exposed functions. Each cell type, namely, \cppLstinline{Vertex}, \cppLstinline{Halfedge}, or \cppLstinline{Face}, can be extended independently, which implies that there are eight plausible combinations that the user can select from to form the final DCEL type of the arrangement.

Extending the arrangement features is useful for many applications, but essential for applications that compute the overlay of arrangements as discussed in the next Section.

% Add a discussion about extending the triangulation data structure in 2D and 3D
% Change the title to be more general to reflect other extensions

% -----------------------------------------------------------------------------
\subsection{Arrangement Overlay Traits}
\label{sec:code:overlay}
% -----------------------------------------------------------------------------
The map overlay of two arrangements $\calA_1$ and $\calA_2$, conveniently referred to as the \textcolor{red}{red} and \textcolor{blue}{blue} arrangements, is a third arrangement $\calA$, such that there is a cell $c$ in $\calA$ iff there are cells $c_1$ and $c_2$ in $\calA_1$ and $\calA_2$, respectively, and $c$ is a maximal connected component of $c_1 \cap c_2$.
% Arrangements are subdivisions of some ambient space (see Section~\ref{ssec:modules:aos2})
Computing the overlay of two arrangements is useful for many applications, including Boolean operations; see Section~\ref{ssec:modules:bso2}. Indeed, the \iiDArrangementsPackage{} package provides function templates that computes the overlay of two arrangements, namely overloaded \cppLstinline{CGAL::overlay()}. In particular, the call \cppLstinline{CGAL::overlay(arr_r, arr_b, arr)} computes the overlay of the arrangements \cppLstinline{arr_r} and \cppLstinline{arr_b} and stores the result in the arrangement \cppLstinline{arr}. All three types must be instances of the \cppLstinline{Arrangement_2<Traits, Dcel>} class template; see Section~\ref{ssec:modules:aos2}. When the function is used in pure C++ code, the geometry-traits classes that substitute the \cppLstinline{Traits} template parameters of the input arrangements must be convertible to the geometry-traits class of the resulting arrangement. We only wrap instances of the overlay function with Python bindings, where all three arrangements use the exact same geometry-traits classes and the same DCEL structures, and thus the types of the three arrangements of the exposed \cppLstinline{CGAL::overlay()} function are identical.

The \cppLstinline{CGAL::overlay()} function template is overloaded with a variant that accepts four arguments. The last argument, referred to as the overlay traits, enables the update of cells of the output arrangement, and in particular their properties. Using the overlay traits is typically accompanied with the extension of one or more types of the arrangement cells that hold the properties. The overlay traits must model the \cppLstinline{OverlayTraits} concept, which requires the provision of ten functions that handle all possible overlapping cases as listed below. Let $v_r$, $e_r$, and $f_r$ denote input \textcolor{red}{red} cells, i.e.,~a vertex, an edge, and a face, respectively, $v_b$, $e_b$, and $f_b$ denote input \textcolor{blue}{blue} cells, and $v$, $e$, and $f$ denote output
cells.
\begin{compactenum}
\item A new vertex $v$ is induced by coinciding vertices $v_r$ and $v_b$.
\item A new vertex $v$ is induced by a vertex $v_r$ that lies on an edge $e_b$.
\item An analogous case of a vertex $v_b$ that lies on an edge $e_r$.
\item A new vertex $v$ is induced by a vertex $v_r$ that is contained in a face $f_b$.
\item An analogous case of a vertex $v_b$ contained in a face $f_r$.
\item A new vertex $v$ is induced by the intersection of two edges $e_r$ and $e_b$.
\item A new edge $e$ is induced by the (possibly partial) overlap of two edges $e_r$ and $e_b$.
\item A new edge $e$ is induced by the an edge $e_r$ that is contained in a face $f_b$.
\item An analogous case of an edge $e_b$ contained in a face $f_r$.
\item A new face $f$ is induced by the overlap of two faces $f_r$ and $f_b$.
\end{compactenum}

Evidently a custom C++ overlay traits cannot be defined in Python; more precisely, the traits type must be known when the bindings are compiled. We introduce and expose with Python bindings two models of the \cppLstinline{OverlayTraits} concept. The most general between the two, called \cppLstinline{Arr_overlay_traits}, defines ten functions that correspond to the list above, each accepting three arguments, namely, two objects that represent input cells, and one object that represents an output cell. By default these functions do nothing. A user (that is, a Python programmer) can override any subset of these functions. One constructor of this model accepts all the ten functions at once. Another constructor accepts a single function, which corresponds to Function (10) in the list above.

In the following we assume that the face type of the arrangement
% \cppLstinline{Arrangement_2} instance
is extended. The code excerpt in Listing~\ref{lst:twoFaceExtend} constructs two arrangements with two faces each. For each arrangement the properties of the unbounded face and the bounded face are initialized with Python integer objects~$0$ and~$1$, respectively.
%
The code excerpt in Listing~\ref{lst:overlayTraits} computes the overlay of the two arrangements constructed by the code in Listing~\ref{lst:twoFaceExtend} using the overlay traits. The property of each face of the resulting arrangement is updated as part of the overlay computation to indicate the number of overlapping bounded faces; see Figure~\ref{fig:faceExt}.
%
Observe that while the computation of the overlay is carried out by the compiled C++ code, the summation is carried out by a Python \pyLstinline{lambda} function, which accepts as the third argument the face to be updated. By default, arguments are copied into new Python objects. We pass the new face by reference, overriding the default, to enforce persistent updates.

\begin{lstfloat}
  \def\filename{overlay.py}%
  \lstinputlisting[style=pythonFramedStyle,basicstyle=\normalsize,
                   firstline=14,lastline=37,
                   label={lst:twoFaceExtend},
                   caption={Constructing two arrangements with their faces extended and initializing their data.}]
                  {\pythonDir\filename}
\end{lstfloat}

\begin{lstfloat}
  \begin{lstlisting}[style=pythonFramedStyle,basicstyle=\normalsize,
                     label={lst:overlayTraits},
                     caption={Computing the map overlay of two arrangements using the general overlay traits.}]
traits = Aos2.Arr_overlay_traits(lambda f1,f2,f: f.set_data(f1.data()+f2.data()))
Aos2.overlay(arr1, arr2, result, traits)
  \end{lstlisting}
\end{lstfloat}

\begin{figure}[!htp]
  \captionsetup[subfigure]{justification=centering}
  \centering%
  \subfloat[]{\label{fig:faceExt}
    \begin{tikzpicture}
      \fill[polyALightColor] (0,0) rectangle (2,2);
      \fill[polyBLightColor,opacity=0.5] (1,1) rectangle (3,3);
      \draw[thick,polyADarkColor] (0,0) rectangle (2,2);
      \draw[thick,polyBDarkColor] (1,1) rectangle (3,3);
      \node at (2.5,0.5) {[0]};
      \node at (0.5,0.5) {[1]};
      \node at (2.5,2.5) {[1]};
      \node at (1.5,1.5) {[2]};
      \node[point] at (0,0) {};
      \node[point] at (2,0) {};
      \node[point] at (0,2) {};
      \node[point] at (2,2) {};
      \node[point] at (1,1) {};
      \node[point] at (3,1) {};
      \node[point] at (1,3) {};
      \node[point] at (3,3) {};
      \node[point] at (2,1) {};
      \node[point] at (1,2) {};
    \end{tikzpicture}}\quad\quad
  \subfloat[]{\label{fig:vertexExt}
    \begin{tikzpicture}[scale=0.2]
      \draw[thick,polyADarkColor] (3,4) circle (5);
      \draw[thick,polyADarkColor] (-3,-4) circle (5);
      \draw[thick,polyBDarkColor] (4,-3) circle (5);
      \draw[thick,polyBDarkColor] (-4,3) circle (5);
      \node[point=red!50!white,label={[label distance=-1pt]180:4}] at (-8, -4) {}; % 4
      \node[point=green,label={[label distance=-1pt]180:6}] at (-7, -1) {};        % 6
      \node[point=red!50!white,label={[label distance=-1pt]180:2}] at (-9, 3) {};  % 2
      \node[point=red!50!white,label={[label distance=-1pt]180:4}] at (-2, 4) {};  % 4
      \node[point=green,label={[label distance=-1pt]90:6}] at (-1, 7) {};          % 6
      \node[point=red!50!white,label={[label distance=-1pt]180:2}] at (-1, -3) {}; % 2
      \node[point=blue,label={[label distance=-1pt]0:12}] at (0, 0) {};            % 12
      \node[point=green,label={[label distance=-1pt]-90:6}] at (1, -7) {};         % 6
      \node[point=red!50!white,label={[label distance=-1pt]0:2}] at (1, 3) {};     % 2
      \node[point=red!50!white,label={[label distance=-1pt]0:4}] at (2, -4) {};    % 4
      \node[point=green,label={[label distance=-1pt]0:6}] at (7, 1) {};            % 6
      \node[point=red!50!white,label={[label distance=-1pt]0:4}] at (8, 4) {};     % 4
      \node[point=red!50!white,label={[label distance=-1pt]0:2}] at (9, -3) {};    % 2
    \end{tikzpicture}}
  \caption[]{%
    \subref{fig:faceExt} The arrangement faces are extended with integers that indicate the number of overlapping bounded faces, shown in brackets.
    \subref{fig:vertexExt} The arrangement vertices are extended with integers that indicate the weighted degree of the vertices.}
  \label{fig:extend}
\end{figure}

In many cases, such as in the example above, the property of the new cell depends solely on the properties of the overlapping two cells. To this end we introduce (and expose) a second model of the \cppLstinline{OverlayTraits} concept called \cppLstinline{Arr_overlay_function_traits}. This model also defines ten functions that correspond to the list above. However, here each function accepts the two Python objects that extend the overlapping cells as input arguments and returns the Python object that extends the resulting cell. The code excerpt in Listing~\ref{lst:overlayFunctionTraits} has the same effect the code in Listing~\ref{lst:overlayTraits} has, but is more compact.

\begin{lstfloat}
  \begin{lstlisting}[style=pythonFramedStyle,basicstyle=\normalsize,
                     label={lst:overlayFunctionTraits},
                     caption={Computing the map overlay of two arrangements using the functional overlay traits.}]
traits = Aos2.Arr_overlay_function_traits(lambda x, y: x+y)
os2.overlay(arr1, arr2, result, traits)
  \end{lstlisting}
\end{lstfloat}

Each one of the ten functions supported by the \cppLstinline{Arr_overlay_function_traits} model returns a Python object that is passed back to the compiled C++ code. Then, the object is stored with the new cell. Thus, there is no need to pass arguments by reference (even though it could be more efficient in certain cases); however, the implementation of this model presents a new coding challenge---if a certain cell is not extended, attempting to access its non-existing extension would cause a compilation error.
%
Assume that only the vertex type of the \cppLstinline{Arrangement_2} instance is extended. The Python code excerpt in Listing~\ref{lst::overlayCircleSegment} computes the overlay of two arrangements and updates the property of each vertex of the resulting arrangement to indicate the weighted degree of the vertex, where blue incident edges weigh twice as much as red incident edges; see Figure~\ref{fig:vertexExt}. We set all the six functions that update output vertices in the \cppLstinline{Arr_overlay_function_traits} object using dedicated setters. The name of a setter matches the pattern \lstinline[language={C++},mathescape=true,columns=fixed]{set_$c_rc_b$_$c$()}, where each of $c_r$, $c_b$, and $c$ can be substituted with \cppLstinline{v}, \cppLstinline{e}, or \cppLstinline{f}. $c_r$ and $c_b$ determine the input red and blue cell types, respectively, and $c$ determines the output cell type.

\begin{lstfloat}
  \begin{lstlisting}[style=pythonFramedStyle,basicstyle=\normalsize,
                     label={lst::overlayCircleSegment},
                     caption={Constructing two arrangements with their vertices extended and computing their map overlay using the overlay function traits.}]
Aos2.insert(arr1,[Curve(Circle(Point(3,4),25)),Curve(Circle(Point(-3,-4),25))])
Aos2.insert(arr2, [Curve(Circle(Point(3,4),25)), Curve(Circle(Point(3,4),25))])
for arr in [arr1, arr2]:
  for v in arr.vertices():
    v.set_data(v.degree())
traits = Aos2.Arr_overlay_function_traits()
traits.set_vv_v(lambda x, y: 2*x+y)
traits.set_ve_v(lambda x, y: 2*x+2)
traits.set_vf_v(lambda x, y: 2*x)
traits.set_ev_v(lambda x, y: 4+y)
traits.set_fv_v(lambda x, y: y)
traits.set_ee_v(lambda x, y: 6)
Aos2.overlay(arr1, arr2, result, traits)
  \end{lstlisting}
\end{lstfloat}

Consider a generic function called \cppLstinline{apply()} that accepts two objects that represent input cells, namely \cppLstinline{r} and \cppLstinline{b}, one object that represents an output cell, namely \cppLstinline{o}, and a function called \cppLstinline{f}. The objective of \cppLstinline{apply()} is to apply \cppLstinline{f} to the properties of the cells \cppLstinline{r} and \cppLstinline{b} and store the return value as the property of the cell \cppLstinline{o}. Recall that a property of a cell \cppLstinline{c} is obtained and set via the calls \cppLstinline{c.data()} and \cppLstinline{c.set_data()}, respectively. If the type of the output cell is not extended, however, \cppLstinline{apply()} should become idle. Similarly, if the type of an input cell is not extended, the \pyLstinline{None} Python object (represented by \cppLstinline{py::object}) should be passed to \cppLstinline{f} instead. We use SFINAE yet again, twice, to address the above. First, we introduce an overload of \cppLstinline{apply()} that is idle and serves as a fall-through; see Line~9 in Listing~\ref{lst:data}. When a call to \cppLstinline{apply()} is made, the idle overload is selected by the overload resolution process if the output cell does not have a member called \cppLstinline{set_data()}. If the output cell does have this member the other implementation is selected and calls \cppLstinline{data(r)} and \cppLstinline{data(b)} to obtain the properties of the \textcolor{red}{red} and \textcolor{blue}{blue} input cells, respectively. Second, we introduce an overload of \cppLstinline{data()} that serves as a fall-through (Line~2). It does nothing but return the \pyLstinline{None} Python object. It is selected if the corresponding cell does not have a member called \cppLstinline{data()}. If the cell does have this member the other implementation is selected; it returns the property of the cell.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,
                     label={lst:data},
                     caption={Automatic generation of bindings for the overlay function traits exploiting SFINAE.}]
// Fall-through; A::data() does not exist
template <typename A> py::object data(...) { return py::none(); }

// A::data() exists
template <typename A, typename = decltype(std::declval<A>().data())>
const py::object& data(const A* a) { return a->data(); }

// Fall-through; O::set_data() does not exist
template <typename R, typename B, typename O, typename F> void apply(...) {}

// O::set_data() does exist
template <typename R, typename B, typename O, typename F,
          typename =
            decltype(std::declval<O>().set_data(std::declval<typename O::Data>()))>
void apply(const R* r, const B* b, O* o, F f) {
  o->set_data(f(data<R>(r), data<B>(b)));
}
  \end{lstlisting}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsection{Miscellaneous}
\label{sec:code:misc}
% -----------------------------------------------------------------------------
In this section we list additional techniques used by the binding code.

% -----------------------------------------------------------------------------
\subsubsection{Handle, iterators, and Circulators}
\label{sec:code:misc:iters}
% -----------------------------------------------------------------------------
The \cppLstinline{Handle} concept, provided by the \HandlesandCirculatorsPackage{} package~\cite{cgal:dksy-hc-22}, describes types that are akin to pointers to objects. A handle provides the dereference operator (\cppLstinline{operator*()}) and the member access operator (\cppLstinline{->()}). Since Python does not have any kind of pointers, both a handle to an object in \cgal{} and the object itself are converted to the same Python object. For example, both types \cppLstinline{Arrangement_2::Vertex} and \cppLstinline{Arrangement_2::Vertex_handle} are converted to the Python type \pyLstinline{Vertex}, which is an attribute of the Python type \pyLstinline{Arrangement_2}.

The \cppLstinline{Iterator} concept and its refinements describe types that can be used to identify and traverse the elements of container that contains sequential data.\footnote{For more information about STL iterators, see, e.g., \url{https://en.cppreference.com/w/cpp/iterator}.} An iterator provides the increment or decrement operators. In \cgal{} quite often an iterator is convertible to a handle, for example, \cppLstinline{Arrangement_2::Vertex_iterator} is convertible to \cppLstinline{Arrangement_2::Vertex_handle}. Therefore, also \cppLstinline{Arrangement_2::Vertex_iterator} is converted to the python class \pyLstinline{Vertex}. Every converted iterator is supplied with both magic functions \pyLstinline{__iter__} and \pyLstinline{__next__}, thus made a \emph{Python iterator}.\footnote{For more information about Python iterators, see, e.g., \url{https://docs.python.org/3/c-api/iterator.html}.} The \pyLstinline{__iter__} function simply returns the input object, and the \pyLstinline{__next__} function returns the next object in the traversal order of the corresponding iterator.

Similar to the \cppLstinline{Iterator} concept and its refinements, the \cppLstinline{Circulator} concept and its refinements, also provided by the \HandlesandCirculatorsPackage{} package, describe types that can be used to identify and traverse the elements of container that contains circular data, for example, the halfedges incident to a face or the halfedges incident to a vertex in an arrangement.  A circulator object does not have a past-the-end value. Instead, the range $[a, b)$ of two circulators $a$ and $b$ denotes either the empty range, or the sequence of all elements in the container. nanobind supports several features that aid in the wrapping if iterators. Circulators are artificially converted to iterators to leverage on those features. In addition, while traversing a circulator, an stop-iteration exception is thrown when a circular refers to an item that has been traversed already.

% -----------------------------------------------------------------------------
\subsubsection{Functions Accepting Collections of Elements}
\label{sec:code:input}
% -----------------------------------------------------------------------------
The Standard Template Library (STL) provides various type-safe containers for storing collections of related objects. The \cppLstinline{Container} concept describes types of objects that store collections of other objects (their elements).\footnote{For more   information about STL containers, see, e.g.,   \url{https://en.cppreference.com/w/cpp/container}.} Container models are implemented as class templates, which enables great flexibility in the elements types and in the implemented algorithms that operate on container objects. Traditionally, implementations of algorithms in C++ manipulate iterators pointing into the containers they operate on. To date it is popular to pass a collection of elements to a function via two generic input iterators, where the first points at the first element of a container and the second points past the end of the container. An input iterator object, the type of which is a model of the the \cppLstinline{InputIterator} concept,\footnote{For more information about input iterators, see, e.g.,   \url{https://en.cppreference.com/w/cpp/iterator/input_iterator}.} supports reading from the location obtained via the dereference operator and can be pre- and post incremented.  The Boost.Range library provides an alternative modern method, which uses \emph{ranges}, for applying algorithms on collections of objects. In particular, it utilizes a new family of concepts that refine a basic concept called \cppLstinline{Range}. The \cppLstinline{Range} concept is similar to the \cppLstinline{Container} concept; it requires the provision of iterators for accessing a half-open range of elements and provides information about the number of elements in the range. The new method results in code that is more efficient and more expressive (and thus more comprehensible).\footnote{See   \url{https://www.boost.org/doc/libs/1_78_0/libs/range/doc/html/index.html} for the documentation of Boost.Range.}  Soon, (C++20) ranges will become part of the standard.\footnote{For more information about STL ranges, see, e.g., \url{https://en.cppreference.com/w/cpp/ranges}.} The \HandlesandCirculatorsPackage{} package of \cgal{} provides a variant of a \cppLstinline{Range} concept suitable for \cgal{}. Many functions in \cgal{} accept as input collections of elements, and some of them already use this concept. The use of ranges is expected to grow. For every function in \cgal{} that operates on one or more collections of elements, and regardless of the interface of the function, that is, whether a pair of generic input iterators, or a range, is used to represent each collection, we introduce and expose a wrapper function that accepts a Python list (of type \cppLstinline{py::list}) as an argument;\footnote{For more information on Python lists, see, e.g.,   \url{https://docs.python.org/3/tutorial/datastructures.html\#more-on-lists}.} the wrapper function calls the original function, properly passing the input collection; see Listing~\ref{lst:insert} for an example of such a function that uses iterators; the wrapper function is shown in Listing~\ref{lst:insertWrapper}; an excerpt code in Python that exploits the above is shown in Listing~\ref{lst:insertPython}. The function \cppLstinline{insert_curves()} (in Listing~\ref{lst:insertWrapper}) exploits an iterator adapter called \cppLstinline{stl_input_iterator}

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:insert},%
                     caption={The signature of the free function that inserts a collections of curves into an arrangement.}]
template <typename InputIterator>
CGAL::insert(Arrangement_2& arr, InputIterator first, InputIterator past_the_end)
  \end{lstlisting}
\end{lstfloat}

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:insertWrapper},%
                     caption={A function that wraps the function shown in Listing~\ref{lst:insert} and accepts a Python list that contains the input curves.}]
void insert_curves(Arrangement_2& arr, py::list& lst) {
  if (! lst) return;
  if (py::isinstance<X_monotone_curve_2>(lst[0]).check()) {
    auto begin = stl_input_iterator<X_monotone_curve_2>(lst);
    auto end = stl_input_iterator<X_monotone_curve_2>();
    CGAL::insert(arr, begin, end);
  }
  else if (py::isinstance<Curve_2>(lst[0]).check()) {
    auto begin = stl_input_iterator<Curve_2>(lst);
    auto end = stl_input_iterator<Curve_2>();
    CGAL::insert(arr, begin, end);
  }
}
  \end{lstlisting}
\end{lstfloat}

\begin{lstfloat}
  \begin{lstlisting}[style=pythonFramedStyle,basicstyle=\normalsize,%
                     label={lst:insertPython},%
                     caption={A code sample in Python that inserts three curves into an arrangement.}]
arr = Arrangement_2()
c1 = X_monotone_curve_2(Point_2(0, 0), Point_2(1, 0))
c2 = X_monotone_curve_2(Point_2(1, 0), Point_2(0, 1))
c3 = X_monotone_curve_2(Point_2(0, 1), Point_2(1, 1))
Aos2.insert(arr, [c1, c2, c3])
  \end{lstlisting}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsubsection{Functions Resulting in Collections of Elements}
\label{sec:code:output}
% -----------------------------------------------------------------------------
Functions may compute collections of elements as results. Using output iterators enables an efficient and flexible method for passing output collections from functions. An output iterator object, the type of which is a model of the the \cppLstinline{OutputIterator} concept,\footnote{For more information of output iterators, see, e.g.,   \url{https://en.cppreference.com/w/cpp/iterator/output_iterator}.} supports writing to the location obtained by the dereference operator and can be pre- and post-incremented. A function that computes a collection of elements accepts an output iterator as an argument and populates the underlying collection. Modern C++ compilers support the efficient transfer of resources from one object of a certain type to another object of the same type, referred to as \emph{move semantics}.\footnote{For more information of move semantics, see, e.g.,   \url{https://en.cppreference.com/w/cpp/language/move_constructor}.} If the underlying collection supports move semantics, a function that computes a collection of elements can simply return the collection, resulting in an elegant yet efficient code. For every function in \cgal{} that results in a collection of elements, and regardless of the interface of the function, that is, whether an output iterator is used or the collection is returned, we introduce and expose a wrapper function that returns a Python list (of type \cppLstinline{py::list}); the wrapper function calls the original function, properly populating a Python list with the output collection, and finally it returns the list.

The free function template \cppLstinline{CGAL::decompose()} accepts an arrangement $\mathcal{A}$ and computes a collection of polymorphic elements via an output iterator. For each vertex $v$ of $\mathcal{A}$ the output collection contains a pair of features---one that directly lies below $v$ and another that directly lies above $v$. Let $v$ be a vertex of $\mathcal{A}$. The feature above (respectively below) $v$
may be one of the following:
\begin{compactitem}
\item Another vertex $u$ having the same $x$-coordinate as $v$.
\item An arrangement edge associated with an $x$-monotone curve that contains $v$ in its $x$-range.
\item An unbounded face in case $v$ is incident to an unbounded face, and there is no curve lying above (respectively below) it.
\item An empty object, in case $v$ is the lower (respectively upper) endpoint of a vertical edge in the arrangement.
\end{compactitem}
Listing~\ref{lst:decompose} shows the signature of the function. Dereferencing the output iterator must yield an object the type of which is \cppLstinline{Decompose_result} shown in Line~2 of Listing~\ref{lst:decomposeWrapper}.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:decompose},%
                     caption={The signature of the free function that decomposes an arrangement into pseudo trapezoids.}]
template <typename OutputIterator>
CGAL::decompose(Arrangement_2& arr, OutputIterator oi);
  \end{lstlisting}
\end{lstfloat}

The wrapper of the \cppLstinline{CGAL::decompose()} template function, shown in Listing~\ref{lst:decomposeWrapper}, returns a list of Python elements; each element is a Python tuple of two items; the first wraps a C++ vertex and the second wraps another Python tuple of two items; the first is the cell above the vertex or \pyLstinline{py::Object} if none exists and the second is the cell below the vertex or \pyLstinline{py::Object} is none exists. Implementing such a wrapper can be done, for example, by introducing an intermediate standard container, say \cppLstinline{container}, and populating it with the elements, of the \cppLstinline{Decompose_result} polymorphic type, computed by the \cppLstinline{CGAL::decompose()} function in C++ (by passing an object of type \cppLstinline{std::back_insert_iterator<Decompose_result>} obtained by the call \cppLstinline{std::back_inserter(container)}, as the output iterator argument of the function), and then transforming the container elements into Python elements. Clearly, this is inefficient. Instead, we use the Boost c++ \pyLstinline{function_output_iterator<>} adapter to directly populate a Python list instead of an intermediate container. The adapter (i) utilizes a helper function called \cppLstinline{decompose_helper()} (not listed), which is applied to every resulting element transforming it to the corresponding bounded Python object, and (ii) appends the latter to the output Python list.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:decomposeWrapper},%
                     caption={A function that wraps the function shown in Listing~\ref{lst:decompose} and returns a Python list that represents a vertical decomposition.}]
py::list decompose(Arrangement_2& arr) {
  using Decompose_result = std::pair<Arrangement_2::Vertex_const_handle,
                                     std::pair<boost::optional<variant>,
                                               boost::optional<variant>>>;
  // The argument type of boost::function_output_iterator (UnaryFunction) must
  // be Assignable and Copy Constructible; hence the application of std::ref().
  auto it = boost::make_function_output_iterator(std::ref(op));
  CGAL::decompose(arr, it);
  return lst;
}
  \end{lstlisting}
\end{lstfloat}

The Python code example shown in Listing~\ref{lst:py:decompose} exploits the above and computes the vertical decomposition shown in Figure~\ref{fig:decompose}.

%% The output:
%% 0 0
%%   unbounded face
%%   unbounded face
%% 2 0
%%   unbounded face
%%    0 0 3 3
%% 3 3
%%    2 0 4 2
%%   unbounded face
%% 4 2
%%   unbounded face
%%   unbounded face
%% 5 3
%%    4 2 6 0
%%   unbounded face
%% 6 0
%%   unbounded face
%%    5 3 8 0
%% 8 0
%%   unbounded face
%%   unbounded face

\begin{lstfloat}
  \def\filename{vertical_decomposition.py}%
  \lstinputlisting[style=pythonFramedStyle,basicstyle=\normalsize,%
                   label={lst:py:decompose},%
                   firstline=15,
                   caption={A code sample in Python that decomposes an
                     arrangement.}]
                  {\pythonDir\filename}
\end{lstfloat}

\begin{figure}[!htp]
  \centerline{%
    \begin{tikzpicture}
      \draw node[point=white] (x) at (4,2) {};
      %
      \draw node[point] (u1) at (0,0) {};
      \draw node[point=cyan] (u2) at (2,2) {};
      \draw node[point] (u3) at (3,3) {};
      \draw node[point=cyan] (u4) at (5,1) {};
      \draw node[point] (u5) at (6,0) {};
      \draw[blue,thick] (u1)--(u2)--(u3)--(x)--(u4)--(u5);
      %
      \draw node[point] (v1) at (2,0) {};
      \draw node[point=cyan] (v2) at (3,1) {};
      \draw node[point] (v3) at (5,3) {};
      \draw node[point=cyan] (v4) at (6,2) {};
      \draw node[point] (v5) at (8,0) {};
      \draw[blue,thick] (v1)--(v2)--(x)--(v3)--(v4)--(v5);
      %
      \draw[dots=10 per 1cm,very thick] (0,-1)--(u1)--(0,4);
      \draw[dots=10 per 1cm,very thick] (2,-1)--(v1)--(u2)--(2,4);
      \draw[dots=10 per 1cm,very thick] (3,-1)--(v2)--(u3)--(3,4);
      \draw[dots=10 per 1cm,very thick] (4,-1)--(x)--(4,4);
      \draw[dots=10 per 1cm,very thick] (5,-1)--(u4)--(v3)--(5,4);
      \draw[dots=10 per 1cm,very thick] (6,-1)--(u5)--(v4)--(6,4);
      \draw[dots=10 per 1cm,very thick] (8,-1)--(v5)--(8,4);
    \end{tikzpicture}}
  \caption{An arrangement of four line segments and its vertical decomposition into pseudo trapezoids, as constructed by the Python code shown in Listing~\ref{lst:py:decompose}.  The segments of the arrangement are drawn in solid blue lines and the segments of the vertical decomposition are drawn in dark dotted lines.}
  \label{fig:decompose}
\end{figure}

%% % -----------------------------------------------------------------------------
%% \subsection{\myLstinline{Python_distance}}
%% \label{sec:code:distance}
%% % -----------------------------------------------------------------------------
%% Similarly to overlay traits, a user may want to define a custom
%% distance class to use with search queries. Here too, as defining a new
%% C++ class is not possible from python, we provide a similar solution:
%% A \myLstinline{Python_distance} class is exposed, which is a model of
%% \myLstinline{GeneralDistance}
%% concept. \url{https://doc.cgal.org/5.2/Spatial_searching/classGeneralDistance.html}
%% It expects 5 functions in its constructor, and those are saved as
%% class members and are used for the respective 5 operations [the
%%   optional are not included] of the concept.

%% Making some things more pythonic:

%% (the extended arrangement data type) Those 10 functions are saved as
%% class members and are then called in the respective 10 [overloaded]
%% versions of \myLstinline{create_vertex}, \myLstinline{create_edge},
%% \myLstinline{create_face object}) (the matching is done by the order
%% of the passed functions and the order of the [overloaded] versions in
%% the official concept reference).

%% This way the user can still define the way the result face/edge/vertex
%% data will be calculated.


==> submission/extenders.tex <==
% =============================================================================
\section{Extenders}
\label{sec:extenders}
% =============================================================================
In several places in our binding code we are given a type that models certain concepts and based on several conditions, this type must be replaced with a new type that models additional concepts. Instead of using old style code in the form of \cppLstinline{#if,#elif,#else,#endif} directives, we exploit generic programming and implement these extenders using modern code that is type safe. In the following we present four such scenarios.

% -----------------------------------------------------------------------------
\subsection{2D Arrangement Traits Extender}
\label{sec:extenders:arrTraits}
% -----------------------------------------------------------------------------
When the user enables the generation of bindings for the \iiDArrangementsPackage{} package, the binding for an instance of the class template \cppLstinline{Arrangement_2<Traits, Dcel>} is generated. When this class template is instantiated the \cppLstinline{Traits} template parameter must be substituted with a specific traits model. By default an instance of the \cppLstinline{Arr_segment_traits_2<Kernel>} is used; however, the user can override this selection and choose any one of the supported geometry traits. We refer to this traits as the basic geometry traits. If the user also enables the generation of bindings for the
\iiDRegularizedBooleanSetOperationsPackage{} package, the basic traits must be extended, because it must also model the \cppLstinline{GeneralPolygonSetTraits_2} concept (see Figure~\ref{fig:atc:gps}); see Section~\ref{ssec:modules:aos2}. The extension however differs for different basic traits. It is automatically done via a dedicated class template and four specializations shown in Listing~\ref{lst:arrTraitsExtender}. The final traits is obtained using this extender as shown in Listing~\ref{lst:arrFinalTraits}. Here,
\cppLstinline{boolean_set_operations_2_bindings()} is a constant binary function (evaluated at compile time) that determines whether the generation of bindings for the
\iiDRegularizedBooleanSetOperationsPackage{} package is enabled, and
\cppLstinline{BGT} is the basic geometry traits.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrTraitsExtender},%
                     caption={2D Arrangement Traits Extender.}]
// Traits extender
template <bool b, typename Base> struct Tr {};

// Specialization for the case where bindings for Bso2 are not generated
template <typename Base>
struct Tr<false, Base> { typedef Base type; };

// Specialization for the general case where bindings for Bso2 are generated
template <typename Base>
struct Tr<true, Base> { typedef CGAL::Gps_traits_2<Base> type; };

// Specialization for the segment traits
template <>
struct Tr<true, CGAL::Arr_segment_traits_2<Kernel>> {
  typedef CGAL::Gps_segment_traits_2<Kernel, Point_2_container> type;
};

// Specialization for the circle segment traits
template <>
struct Tr<true, CGAL::Arr_circle_segment_traits_2<Kernel>> {
  typedef CGAL::Gps_circle_segment_traits_2<Kernel> type;
};
  \end{lstlisting}
\end{lstfloat}

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrFinalTraits},%
                     caption={The final 2D Arrangement traits type definition.}]
typedef Tr<boolean_set_operations_2_bindings(), BGT>::type      Geometry_traits;
  \end{lstlisting}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsection{2D Arrangement DCEL Cell Extenders}
\label{sec:extenders:arrDcel}
% -----------------------------------------------------------------------------
When the user enables the generation of bindings for the \iiDArrangementsPackage{} package, the binding for an instance of the class template \cppLstinline{Arrangement_2<Traits, Dcel>} is generated. When this class template is instantiated the \cppLstinline{Dcel} template-parameter should be substituted with a type that models the \cppLstinline{ArrangementDcel} concept. We substitute this parameter with an instance of the template \cppLstinline{CGAL::Arr_dcel_base<V, H, F>}, where \cppLstinline{V}, \cppLstinline{H}, and \cppLstinline{F} must model the concepts \cppLstinline{ArrangementDcelVertex}, \cppLstinline{ArrangementDcelHalfedge}, and
\cppLstinline{ArrangementDcelFace}, respectively. By default, we substitute these parameters with the instances \cppLstinline{Arr_vertex_base<Traits::Point_2>},
\cppLstinline{Arr_halfedge_base<Traits::X_monotone_curve_2>}, and \cppLstinline{Arr_face_base}, respectively, referred to as the basic types of cells. If the user chooses to extend the vertex type, then we substitute \cppLstinline{V} with the instance \cppLstinline{Arr_extended_ vertex<Vb, py::object>}, where \cppLstinline{Vb}
is the basic vertex type above. This conditional extension is carried out via a dedicated class template and two specializations shown in Listing~\ref{lst:arrDcelVertexExtender}. The final vertex type is obtained using this extender as shown in Listing~\ref{lst:arrFinalVertex}. Here, \cppLstinline{is_vertex_extended()} is a constant binary function that determines whether the user extension of vertices is enabled.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrDcelVertexExtender},%
                     caption={2D Arrangement DCEL user extended vertex type extender.}]
// Vertex extender
template <bool b, typename Vb> struct Vertex_extender {};

// Specialization
template <typename Vb> struct Vertex_extender<false, Vb> { typedef Vb type; };

// Specialization
template <typename Vb> struct Vertex_extender<true>
{ typedef CGAL::Arr_extended_vertex<Vb, py::object> type; };
  \end{lstlisting}
\end{lstfloat}

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrFinalVertex},%
                     caption={The final 2D Arrangement vertex type definition.}]
CGAL::Arr_vertex_base<Geometry_traits::Point_2>                         Vb;
typedef Vertex_extended<is_vertex_extended(), Vb, py::object>::type     V;
  \end{lstlisting}
\end{lstfloat}

If the user also enables the generation of bindings for the \iiDRegularizedBooleanSetOperationsPackage{} package, the template parameters \cppLstinline{H} and \cppLstinline{F} must be substituted with types that also model the
\cppLstinline{GeneralPolygonSetDcelHalfedge} and \cppLstinline{GeneralPolygonSetDcelFace} concepts, respectively; see Section~\ref{ssec:modules:bso2}. In addition, similar to the case of vertex extension, if the user chooses to extend the halfedge or face types, then we substitute \cppLstinline{V} with the instances \cppLstinline{Arr_extended_halfedge<Hb, py::object>} or \cppLstinline{Arr_extended_ face<Fb, py::object>}, respectively, where
\cppLstinline{Hb} and \cppLstinline{Fb} are the types above. The conditional extensions of the halfedge type are carried out via dedicated class templates and corresponding specializations shown in Listing~\ref{lst:arrDcelBasicHalfedgeExtender} and
Listing~\ref{lst:arrDcelHalfedgeExtender}. The final halfedge type is obtained using these extenders as shown in Listing~\ref{lst:arrFinalHalfedge}. Here, \cppLstinline{boolean_set_operations_2_bindings()} is a constant binary function that determines whether the generation of bindings for the \iiDRegularizedBooleanSetOperationsPackage{} package is enabled, and \cppLstinline{is_halfedge_extended()} is a constant binary function that determines whether the user extension of halfedges is enabled.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrDcelBasicHalfedgeExtender},%
                     caption={2D Arrangement DCEL Halfedge extender for 2D Regularized Boolean set operations.}]
// Basic halfedge extender
template <bool b> struct Halfedge_gps {};

// Specialization
template <> struct Halfedge_gps<false>
{ typedef CGAL::Arr_halfedge_base<Geometry_traits::X_monotone_curve_2> type; };

// Specialization
template <> struct Halfedge_gps<true>
{ typedef CGAL::Gps_halfedge_base<Geometry_traits::X_monotone_curve_2> type; };
  \end{lstlisting}
\end{lstfloat}

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrDcelHalfedgeExtender},%
                     caption={2D Arrangement DCEL user extended halfedge type extender.}]
// Halfedge extender
template <bool b, typename Hb> struct Halfedge_extender {};

// Specialization
template <typename Hb> struct Halfedge_extender<false, Hb> { typedef Hb type; };

// Specialization
template <typename Hb> struct Halfedge_extender<true, Hb>
{ typedef CGAL::Arr_extended_halfedge<Hb, py::object> type; };
  \end{lstlisting}
\end{lstfloat}

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrFinalHalfedge},%
                     caption={The final 2D Arrangement DCEL halfedge type definition.}]
typedef Halfedge_gps<boolean_set_operations_2_bindings()>::type         Hb;
typedef Halfedge_extended<is_halfedge_extended(), Hb, py::object>::type H;
  \end{lstlisting}
\end{lstfloat}

Similarly, the conditional extensions of the face type are carried out via dedicated class templates and corresponding specializations shown in Listing~\ref{lst:arrDcelBasicFaceExtender} and Listing~\ref{lst:arrDcelFaceExtender}. The final face type is obtained using these extenders as shown in Listing~\ref{lst:arrFinalFace}.
\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrDcelBasicFaceExtender},%
                     caption={2D Arrangement DCEL Face extender for 2D Regularized Boolean set operations.}]
// Basic face extender
template <bool b> struct Face_gps {};

// Specialization
template <> struct Face_gps<false> { typedef CGAL::Arr_face_base type; };

// Specialization
template <> struct Face_gps<true> { typedef CGAL::Gps_face_base type; };
  \end{lstlisting}
\end{lstfloat}

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrDcelFaceExtender},%
                     caption={2D Arrangement DCEL user extended face type extender.}]
// Face extender
template <bool b, typename Fb> struct Face_extender {};

// Specialization
template <typename Fb> struct Face_extender<false, Fb> { typedef Fb type; };

// Specialization
template <typename Fb> struct Face_extender<true, Fb>
{ typedef CGAL::Arr_extended_face<Fb, py::object> type; };
  \end{lstlisting}
\end{lstfloat}

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:arrFinalFace},%
                     caption={The final 2D Arrangement DCEL face type definition.}]
typedef Face_gps<boolean_set_operations_2_bindings()>::type             Fb;
typedef Face_extended<is_face_extended(), Fb, py::object>::type         F;
  \end{lstlisting}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsection{2D Triangulation Cell Extenders}
\label{sec:extenders:iitri}
% -----------------------------------------------------------------------------
When the user enables the generation of bindings for the \iiDTriangulationsPackage{} package, the binding for an instance of one of the 2D triangulation class templates is generated. Each of these class templates has a template parameter that must be substituted with a model of the concept \cppLstinline{TriangulationDataStructure_2} when the triangulation class template is instantiated. We substitute this parameter with an instance of the class template \cppLstinline{Triangulation_data_structure_2<V, F>}.

The type that substitutes the \cppLstinline{V} template parameter when the class template \cppLstinline{Triangulation_data_structure_ 2<V, F>} is instantiated must model the \cppLstinline{TriangulationDSVertexBase_2} concepts. If the binding is generated for a periodic triangulation, this parameter must be substituted with a type that also models the concept \cppLstinline{Periodic_2TriangulationDSVertexBase_2}. The extension is
automatically done via a dedicated class template and three specializations shown in Listing~\ref{lst:iitriBaseVertexExtender}. Here \cppLstinline{Traits} is the geometry traits type; see Section~\ref{ssec:modules:tri2} for an explanation on how this type is
determined.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:iitriBaseVertexExtender},%
                     caption={The 2D Triangulation base vertex type extender.}]
// Vertex base selection
template <bool b, int i> struct Vertex_base_name {};

// Specialization
template <int i> struct Vertex_base_name<false, i>
{ typedef CGAL::Triangulation_vertex_base_2<Traits> type; };

// Specialization
template <> struct Vertex_base_name<false, CGALPY_TRI2_REGULAR>
{ typedef CGAL::Regular_triangulation_vertex_base_2<Traits> type; };

// Specialization
template <int i> struct Vertex_base_name<true, i>
{ typedef CGAL::Periodic_2_triangulation_vertex_base_2<Traits> type; };
  \end{lstlisting}
\end{lstfloat}

If the user chooses to extend the vertex type, the type that substitutes the \cppLstinline{V} template parameter is further extended. This is automatically done via yet another dedicated class template and two specializations shown in Listing~\ref{lst:iitriExtendedVertexExtender}.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:iitriExtendedVertexExtender},%
                     caption={The 2D Triangulation user extended vertex type extender.}]
// Vertex with info
template <bool b, typename Vb> struct Vertex_with_info {};

// Specialization
template <typename Vb> struct Vertex_with_info<false, Vb> { typedef Vb type; };

// Specialization
template <typename Vb> struct Vertex_with_info<true, Vb>
{ typedef CGAL::Triangulation_vertex_base_with_info_2<py::object, Traits, Vb> type; };
  \end{lstlisting}
\end{lstfloat}

If the triangulation is used to define an alpha shape type, the template
parameter \cppLstinline{V} must be substituted with a type that also models
the concept \cppLstinline{AlphaShapeVertex_2}; see
Section~\ref{ssec:modules:as2}. This is automatically done via yet another
class template shown in Listing~\ref{lst:iitriASVertexExtender}.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:iitriASVertexExtender},%
                     caption={The 2D Triangulation for alpha shapes vertex type extender.}]
// Vertex alpha shape
template <bool b, typename Vb, typename ExactComparison>
struct Vertex_alpha_shape {};

// Specialization
template <typename Vb, typename ExactComparison>
struct Vertex_alpha_shape<false, Vb, ExactComparison> { typedef Vb type; };

// Specialization
template <typename Vb, typename ExactComparison>
struct Vertex_alpha_shape<true, Vb, ExactComparison>
{ typedef CGAL::Alpha_shape_vertex_base_2<Traits, Vb, ExactComparison> type; };
  \end{lstlisting}
\end{lstfloat}

Finally, if the binding is generated for a hierarchy triangulation, e.g., an instance of the template parameter \cppLstinline{Triangulation_hierarchy_2<Triangulation_2>}, the
\cppLstinline{V} template parameter must be substituted with a type that also models the concept \cppLstinline{TriangulationHierarchyVertexBase_2}. (Observe that there is no special requirements on the type that substitutes the \cppLstinline{F} parameter in this case.) This is automatically done via yet another class template shown in Listing~\ref{lst:iitriHierarchyVertexExtender}.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:iitriHierarchyVertexExtender},%
                     caption={The 2D Triangulation hierarchy vertex type extender.}]
// Vertex triangulation hierarchy
template <bool b, typename Vb> struct Vertex_hierarchy {};

// Specialization
template <typename Vb> struct Vertex_hierarchy<false, Vb> { typedef Vb type; };

// Specialization
template <typename Vb> struct Vertex_hierarchy<true, Vb>
{ typedef CGAL::Triangulation_hierarchy_vertex_base_2<Vb> type; };
  \end{lstlisting}
\end{lstfloat}

% Basic
%%%%%%%
The type \cppLstinline{Vb} is defined as the vertex base type.  If bindings are generated for a periodic triangulation, the type \cppLstinline{Vb} is defined as \cppLstinline{Periodic_2_triangulation_vertex_base_2<Traits>}; otherwise, if bindings are generated for an instance of \cppLstinline{Regular_triangulation_2<Traits, Tds>}, the type \cppLstinline{Vb} is defined as \cppLstinline{Regular_triangulation_ vertex_base_2<Traits>}; otherwise, the type \cppLstinline{Vb} is defined as
\cppLstinline{Triangulation_vertex_base_2<Traits>};
% Extended
%%%%%%%%%%
If the user enables vertex-type extension, the type \cppLstinline{Vbi} is defined as
\cppLstinline{Triangulation_vertex_base_with_ info_2<py::object, Kernel, Vb>}; otherwise the type \cppLstinline{Vbi} is defined as \cppLstinline{Vb}.
% Alpha Shape
%%%%%%%%%%%%%
If the triangulation is used to define an alpha shape type, the type \cppLstinline{Vbia} is defined as \cppLstinline{Alpha_shape_vertex_base_2<Traits, Vb, ExactComparison>},
where \cppLstinline{ExactComparison} is substituted with either \cppLstinline{true} or \cppLstinline{false} based on the setting of the \cmake{} flag \cmakeLstinline{CGALPY_AS2_EXACT_COMPARISON}; see Table~\ref{tab:as2}. Otherwise, \cppLstinline{V} is defined as \cppLstinline{Vbi}.
% Hierarchy
%%%%%%%%%%%
If the binding is generated for a hierarchy triangulation, the final vertex type \cppLstinline{V} is defined as \cppLstinline{Triangulation_hierarchy_vertex_ base_2<Vbi>}; otherwise the final vertex type \cppLstinline{V} is defined as \cppLstinline{Vbia}; see Listing~\ref{lst:iitriFinalVertex}. Here, \cppLstinline{is_periodic()}, \cppLstinline{vertex_with_info()}, \cppLstinline{alpha_shape_2_bingings()}, and
\cppLstinline{hierarchy()} are constant binary functions. \cppLstinline{is_periodic()} that determines whether the triangulation, binding for which is generated, is periodic.
\cppLstinline{vertex_with_info()} determines whether the user extension of vertices is enabled. \cppLstinline{alpha_shape_2_bingings()} indicates whether bindings for the \iiDAlphaShapesPackage{} package. \cppLstinline{hierarchy()} indicates whether the binding is generated for a hierarchy triangulation.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:iitriFinalVertex},%
                     caption={The final 2D Triangulation vertex type definition.}]
typedef Vertex_base_name<is_periodic(), CGALPY_TRI2>::type           Vb;
typedef Vertex_with_info<vertex_with_info(), Vb>::type               Vbi;
typedef Vertex_alpha_shape<alpha_shape_2_bindings(), Vbi, Ec>::type  Vbia;
typedef Vertex_hierarchy<hierarchy(), Vbia>::type                    V;
  \end{lstlisting}
\end{lstfloat}

The final face type is determined in a similar fashion. The only difference between the selections of the vertex and face types is that the setting of the \cmake{} flag \cmakeLstinline{CGALPY_TRI2_HIERARCHY} does not have an effect on the face type selection.

% -----------------------------------------------------------------------------
\subsection{3D Triangulation Cell Extenders}
\label{sec:extenders:iiitri}
% -----------------------------------------------------------------------------
When the user enables the generation of bindings for the \iiiDTriangulationsPackage{} package, the binding for an instance of one of the 3D triangulation class templates is generated; see Section~\ref{ssec:modules:tri3}. The scenario here is similar to the scenario of the \iiDTriangulationsPackage{} package described in Section~\ref{sec:extenders:iitri}. We skip the description of the extenders and jump to the description of their application.

If bindings are generated for a periodic triangulation, the type \cppLstinline{Vbp} is defined as \cppLstinline{Periodic_3_triangulation_ ds_vertex_base_3<>}; otherwise, \cppLstinline{Vbp} is defined as \cppLstinline{Triangulation_ds_vertex_base_3<>}.
%
If bindings are generated for an instance of either \cppLstinline{Regular_triangulation_vertex_base_3<Kernel>} or \cppLstinline{Periodic_3_ Regular_triangulation_vertex_base_3<Kernel>}, the type \cppLstinline{Vb} is defined as \cppLstinline{Regular_triangulation_ vertex_base_3<Traits, Vbp>}; otherwise, the type \cppLstinline{Vb} is defined as \cppLstinline{Triangulation_vertex_base_3<Traits, Vbp>}.
%
If the vertex type is extended, the type \cppLstinline{Vbi} is defined as
\cppLstinline{Triangulation_vertex_base_ with_info_3<py::object, Traits, Vb>}; otherwise, the type \cppLstinline{Vbi} is defined as \cppLstinline{Vb}.
%
If the binding is generated for a hierarchy triangulation, the type \cppLstinline{Vbih} is defined as \cppLstinline{Triangulation_hierarchy_vertex_base_3<Vbi>}; otherwise the type \cppLstinline{Vbih} is defined as \cppLstinline{Vbi}.
%
If the triangulation is used to define an alpha shape type, the final type \cppLstinline{V} (that substitutes the \cppLstinline{V} parameter) is defined as either
\cppLstinline{Alpha_shape_vertex_base_3<Traits, Vbih, ExactComparison>}
or
\cppLstinline{Fixed_Alpha_shape_vertex_base_3<Traits, Vbih, ExactComparison>} based on the selection of the alpha shape class (either fixed or plain); see Table~\ref{tab:as3}; \cppLstinline{ExactComparison} is substituted with either \cppLstinline{true} or \cppLstinline{false} based on the user selection of exact comparisons; see Table~\ref{tab:as3}. Otherwise, \cppLstinline{V} is defined as \cppLstinline{Vbih}; see Listing~\ref{lst:iiitriFinalVertex}. (Observe that while 3D periodic regular triangulations are supported in the form of the class template \cppLstinline{Periodic_3_regular_triangulation_3}, corresponding 2D triangulations are not; thus the difference between the structures of the code in Listing~\ref{lst:iitriFinalVertex} and Listing~\ref{lst:iiitriFinalVertex}.

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,%
                     label={lst:iiitriFinalVertex},%
                     caption={The final 3D Triangulation vertex type definition.}]
typedef Vertex_periodic<is_periodic()>::type                         Vb;
typedef Vertex_regular<is_regular(), Vb>::type                       Vbr;
typedef Vertex_with_info<vertex_with_info(), Vbr>::type              Vbri;
typedef Vertex_alpha_shape<alpha_shape_3_bindings(), Vbri, Ec>::type Vbria;
typedef Vertex_hierarchy<hierarchy(), Vbria>::type                   V;
  \end{lstlisting}
\end{lstfloat}

The final cell type is determined in a similar fashion. The only difference between the selections of the vertex and cell types is that the setting of the \cmake{} flag \cmakeLstinline{CGALPY_TRI3_HIERARCHY} does not have an effect on the cell type selection.


==> submission/modules.tex <==
% =============================================================================
\section{Binding Modules}
\label{sec:modules}
% =============================================================================
We describe the bindings generated by our system for various \cgal{}
packages and exemplify the use of the generated bindings.
%
When developing code in Python that uses the bindings, the statement
that imports the binding library, that is,
\begin{lstlisting}[style=pythonStyle]
>>> import CGALPY
\end{lstlisting}
(assuming the default binding library name is retained) must precede
any statement that use the binding. This statement is omitted in all
examples hereafter.

% -----------------------------------------------------------------------------
\subsection{Two- and Three-Dimensional Kernel Bindings}
\label{ssec:modules:kernel}
% -----------------------------------------------------------------------------
The \iiDandiiiDGeometryKernelPackage{}
package~\cite{cgal:bfghhkps-lgk23-22} of \cgal{} consists of constant-size non-modifiable geometric primitive objects and operations on these objects. The objects are sets of points in $d$-dimensional affine Euclidean space, where $d = 2,3$.  Each point is uniquely represented either by Cartesian coordinates or by homogeneous coordinates. An object type can be defined either precatively as a member of a kernel type or imperatively as a global class-template parameterized by a kernel type, defined in the C++ \cppLstinline{CGAL} namespace. For example, assume that \cppLstinline{Kernel} is a kernel type; the type that represents a two-dimensional point of this kernel is either \cppLstinline{Kernel::Point_2} or \cppLstinline{CGAL::Point_2<Kernel>}.  The generated bindings better reflects the latter types; that is, defining a two-dimensional point in Python amounts to the code below.\footnote{When writing code in C++ the precative style is advantageous, as it enables the extension of kernel object types, which is irrelevant when generating bindings.}
\begin{lstlisting}[style=pythonStyle,basicstyle=\normalsize]
>>> Ker = CGALPY.Ker      # define the module namespace
>>> Point_2 = Ker.Point_2 # define the point type in the module namespace
>>> p = Point_2(0, 0);
\end{lstlisting}
Table~\ref{tab:ker} lists the \cmake{} flags associated with the \iiDandiiiDGeometryKernelPackage{} module.  The kernel type is an instance of a chain of C++ class templates. For convenience, \cgal{} provides the following predefined types of generally useful kernels:
\begin{compactenum}
\item \cppLstinline{Exact_predicates_inexact_constructions_kernel}---provides exact geometric predicates, but geometric constructions may be inexact due to round-off errors.
  %
\item
  \cppLstinline{Exact_predicates_exact_constructions_kernel}---provides exact geometric constructions, in addition to exact geometric predicates.
  %
\item
  \cppLstinline{Exact_predicates_exact_constructions_kernel_with_sqrt}---same as \cppLstinline{Exact_predicates_exact _constructions_kernel}, but the number type is a model of the concept that requires operations that perform square roots, namely \cppLstinline{FieldWithSqrt}.\footnote{See
    \url{https://doc.cgal.org/latest/Algebraic_foundations/classFieldWithSqrt.html}.}
  %
\item
  \cppLstinline{Exact_predicates_exact_constructions_kernel_with_kth_root}---same as
  \cppLstinline{Exact_predicates_ exact_constructions_kernel}, but the number type is a model of the concept that requires operations that perform $k$-th roots, namely \cppLstinline{FieldWithKthRoot}.\footnote{See
    \url{https://doc.cgal.org/latest/Algebraic_foundations/classFieldWithKthRoot.html}}
  %
\item \cppLstinline{Exact_predicates_exact_constructions_kernel_with_root_of}---same as
\cppLstinline{Exact_predicates_ exact_constructions_kernel}, but the number type is a model of the concept that requires operations that computes the root of univariate polynomial, namely \cppLstinline{FieldWithRootOf}.\footnote{See \url{https://doc.cgal.org/latest/Algebraic_foundations/classFieldWithRootOf.html}.}
\end{compactenum}

%%%%%%%% Kernel Module Flags
\begin{table}[!htp]
  \caption{\iiDandiiiDGeometryKernelPackage{} module flags}
  \centering\begin{tikzpicture}
  \matrix (first) [tableModuleFlags,
    column 1/.style={nodes={text width=17em}},
    column 2/.style={nodes={text width=3.5em}},
    column 3/.style={nodes={text width=4em}},
    column 4/.style={nodes={text width=23.5em}},
    row 3/.style={nodes={minimum height=2.8em}}
  ] {
    Name & Type & Default & Description\\
    \cmakeLstinline{KERNEL_NAME} & String & \myLstinline{epic} &
      The kernel type used\\
    \cmakeLstinline{KERNEL_INTERSECTION_BINDINGS} & Boolean &
      \myLstinline{true} &
      Determines whether to generate bindings for intersection functions\\
  };
 \end{tikzpicture}
 \label{tab:ker}
\end{table}

All the predefined types are of Cartesian kernels. The \cmake{} flag \cmakeLstinline{CGALPY_KERNEL_NAME} specifies which kernel type should be used for the generated bindings.  Currently, only three predefined types and two specific types are supported; see Table~\ref{tab:ker:name}.

%%%%%%%% Kernel Name Options
\begin{table}[!htp]
  \caption{Kernel name options.}
  \centering\begin{tikzpicture}
    \matrix (first) [tableName,
      column 1/.style={nodes={text width=8em}},
      column 2/.style={nodes={text width=34em}}
    ] {
    \cmakeLstinline{KERNEL_NAME} & Predefined Type\\
    \myLstinline{epic} &
      \cppLstinline{Exact_predicates_inexact_constructions_kernel}\\
    \myLstinline{epec} &
      \cppLstinline{Exact_predicates_exact_constructions_kernel}\\
    \myLstinline{epecws} &
      \cppLstinline{Exact_predicates_exact_constructions_kernel_with_sqrt}\\
   };
 \end{tikzpicture}
   \centering\begin{tikzpicture}
    \matrix (first) [tableName,
      row 2/.append style={nodes={minimum height=2.8em}},
      row 3/.append style={nodes={minimum height=2.8em}},
      column 1/.style={nodes={text width=19em}},
      column 2/.style={nodes={text width=23em}}
    ] {
    \cmakeLstinline{KERNEL_NAME} & Predefined Type\\
    \myLstinline{filteredSimpleCartesianDouble} &
      \setlength{\tabcolsep}{0pt}\renewcommand{\arraystretch}{0}
      \begin{tabular}{l}
        \cppLstinline{NT = double}\\[5pt]
        \cppLstinline{Filtered_kernel<Simple_cartesian<NT>>}
      \end{tabular}\\
    \myLstinline{filteredSimpleCartesianLazyGmpq} &
      \setlength{\tabcolsep}{0pt}\renewcommand{\arraystretch}{0}
      \begin{tabular}{l}
        \cppLstinline{NT = Lazy_exact_nt<Gmpq>}\\[5pt]
        \cppLstinline{Filtered_kernel<Simple_cartesian<NT>>}
      \end{tabular}\\
   };
 \end{tikzpicture}
 \label{tab:ker:name}
\end{table}

The kernel type determines the underlying number type used to represent coefficients and coordinates of kernel objects and for evaluating mathematical expressions that involve these coefficients and coordinates. The Python attribute \pyLstinline{FT}, nested in the Python namespace \pyLstinline{Ker}, exposes the C++ underlying field umber type when it is not a primitive data type; that is, when the selected kernel is nor \cppLstinline{Exact_predicates_inexact_constructions_kernel} neither \cppLstinline{Filtered_kernel<Simple_cartesian<double>>}. (In both cases the underlying number type is \cppLstinline{double}.) Similar to the Python code above, the code below defines a two-dimensional point; here, the coordinates are explicitly converted to the underlying
number type.
\begin{lstlisting}[style=pythonStyle]
>>> p = Point_2(Ker.FT(0), Ker.FT(0))
\end{lstlisting}

The code excerpt shown in Listing~\ref{lst:cmake:epecFixed}, in the \cmake{} language, sets the \cmake{} flags for our first example. When \myLstinline{cmake} is applied with these settings followed by the native build commands (e.g., \bashLstinline{make} on Linux platforms) a library called \myLstinline{CGALPY} is generated. This library consists of the bindings necessary to run the Python example shown in Listing~\ref{lst:py:kerIntersection}, which (i) determines whether two segments intersects, and (ii) computes their intersection point, using the generated binding. Observe that bindings of the \iiDandiiiDGeometryKernelPackage{} module are generated by default, whereas bindings for all other modules must be specifically requested.

\begin{lstfloat}
  \def\filename{epec_fixed_release.cmake}%
  \lstinputlisting[style=cmakeFramedStyle,basicstyle=\normalsize,
                   label={lst:cmake:epecFixed},
                   caption={\cmake{} flag settings used to generate bindings for the exact-predicates and exact-constructions kernel.}]
                  {\cmakeDir\filename}
\end{lstfloat}

\begin{lstfloat}
  \def\filename{ker_intersection.py}%
  \lstinputlisting[style=pythonFramedStyle,basicstyle=\normalsize,
                   firstline=15,
                   label={lst:py:kerIntersection},
                   caption={Computing the intersection between two line segments.}]
                  {\pythonDir\filename}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsection{$d$-Dimensional Kernel Bindings}
\label{ssec:modules:kerneld}
% -----------------------------------------------------------------------------
\cgal{} includes a separate package that consists of constant-size non-modifiable geometric primitive objects in arbitrary dimensions, and operations on these objects, called \dDGeometryKernelPackage{}~\cite{cgal:s-gkd-22}. Similar to the two- and three-dimensional kernels, the objects of the $d$-dimensional kernels are sets of points in some $d$-dimensional affine Euclidean space, where the dimension $d$ is either static across a kernel type or dynamic; see below for more details. Each point is uniquely represented either by Cartesian coordinates or by homogeneous coordinates. For convenience, \cgal{} provides the following
predefined types of generally useful kernels:
\begin{compactenum}
\item \cppLstinline{Epick_d<DimensionTag>}---provides exact geometric predicates, but geometric constructions may be inexact due to round-off errors.
  %
\item \cppLstinline{Epeck_d<DimensionTag>}---provides exact geometric constructions, in addition to exact geometric predicates.
  %
\end{compactenum}
Table~\ref{tab:kerd} lists the \cmake{} flags associated with the \dDGeometryKernelPackage{} module.

%%%%%%%% D Kernel Module Flags
\begin{table}[!htp]
  \caption{\dDGeometryKernelPackage{} module flags}
  \centering\begin{tikzpicture}
  \matrix (first) [tableModuleFlags,
    column 3/.style={nodes={text width=4.5em}},
    column 4/.style={nodes={text width=20.8em}}
  ] {
    Name & Type & Default & Description\\
    \cmakeLstinline{KERNEL_D_NAME} & String & \myLstinline{epicd} &
      The kernel type used\\
     \cmakeLstinline{KERNEL_D_DIMENSION_TAG} & String & dynamic &
      Determines whether the dimension is dynamic\\
    \cmakeLstinline{KERNEL_D_DIMENSION} & Integer & \myLstinline{2} &
      The dimension of the ambient Euclidean space\\
  };
 \end{tikzpicture}
 \label{tab:kerd}
\end{table}

The \cmake{} flag \cmakeLstinline{CGALPY_KERNEL_D_NAME} specifies which kernel type should be used for the generated bindings; see Table~\ref{tab:kerd:name}.

%%%%%%%% D Kernel Name Options
\begin{table}[!htp]
  \caption{$d$-dimensional Kernel name options.}
  \centering\begin{tikzpicture}
  \matrix (first) [tableName, column
    1/.style={nodes={text width=19em}},
    column 2/.style={nodes={text width=30em}}
  ] { \cmakeLstinline{KERNEL_D_NAME} & Predefined Type\\
    \cmakeLstinline{epicd} & \cppLstinline{Epick_d<DimensionTag>}\\
    \cmakeLstinline{epecd} & \cppLstinline{Epeck_d<DimensionTag>}\\
    \cmakeLstinline{cartesiandDouble} & \cppLstinline{Cartesian_d<double>}\\
    \cmakeLstinline{cartesiandLazyGmpq} &
      \cppLstinline{Cartesian_d<Lazy_exact_nt<Gmpq>>}\\
  };
 \end{tikzpicture}
 \label{tab:kerd:name}
\end{table}

When either \cppLstinline{Epick_d<DimensionTag>} or \cppLstinline{Epeck_d<DimensionTag>} are instantiated the template parameter must be substituted with a type that represents the
dimension of the ambient Euclidean space. It may be either \cppLstinline{Dimension_tag<d>} where $d$ is an integer or \cppLstinline{Dynamic_dimension_tag}. In the latter case, the dimension of the space is specified for each point when it is constructed, so it does not need to be known at compile-time of the bindings. The \cmake{} \cmakeLstinline{CGALPY_KERNEL_D_DIMENSION_TAG} flag
specifies whether the dimension is static or dynamic. If it is static, the dimension is extracted from the \cmake{} \cmakeLstinline{CGALPY_KERNEL_D_DIMENSION} \cmake{} flag; ; see
Table~\ref{tab:kerd:dim}.

%%%%%%%% D Kernel Dimension Tag Options
\begin{table}[!htp]
  \caption{$d$-dimensional Kernel dimension tag options.}
  \centering\begin{tikzpicture}
  \matrix (first) [tableName, column
    1/.style={nodes={text width=19em}},
    column 2/.style={nodes={text width=30em}}
  ] { \cmakeLstinline{KERNEL_D_DIMENSION_TAG} & Predefined Type\\
    \cmakeLstinline{static} & \cppLstinline{Dimension_tag<d>}\\
    \cmakeLstinline{dynamic} & \cppLstinline{Dynamic_dimension_tag}\\
  };
 \end{tikzpicture}
 \label{tab:kerd:dim}
\end{table}

The kernel type determines the underlying number type. It is possible to have different underlying number types for the \iiDandiiiDGeometryKernelPackage{} and the \dDGeometryKernelPackage{} models. However, when the number types differ, expensive conversions
might be necessary to combine operations from both kernels, or it may not be possible at all using binding code developed thus far.

The code excerpt in the \cmake{} language shown in Listing~\ref{lst:cmake:cdlg}, sets the \cmake{} flags for our second example. When \myLstinline{cmake} is applied with these settings
followed by the native build commands, a library called \myLstinline{CGALPY_kerdCdlg Dynamic} is generated. This library consists of the bindings necessary to run the Python example shown in
Listing~\ref{lst:py:kerdDoIntersect}, which determines whether two segments in four dimensions intersect using the generated binding.

\begin{lstfloat}
  \def\filename{cdlg_release.cmake}%
  \lstinputlisting[style=cmakeFramedStyle,basicstyle=\normalsize,
                   label={lst:cmake:cdlg},
                   caption={\cmake{} flag settings used to generate bindings for the $d$-dimensional kernel.}]
                  {\cmakeDir\filename}
\end{lstfloat}

\begin{lstfloat}
  \def\filename{kerd_do_intersect.py}%
  \lstinputlisting[style=pythonFramedStyle,basicstyle=\normalsize,
                   firstline=15,
                   label={lst:py:kerdDoIntersect},
                   caption={Determining whether two segments in 4D itersect.}]
                  {\pythonDir\filename}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsection{2D Arrangement Bindings}
\label{ssec:modules:aos2}
% -----------------------------------------------------------------------------
The \cgal{} \emph{arrangements} packages constitute a large component of the \cgal{} library. This component is particularly intricate, partly due to the interplay between combinatorial algorithms and algebra~\cite{fhw-caass-12}. Arrangements are space subdivisions induced by curves and surfaces, which have been intensively studied in discrete and computational geometry~\cite{hs-a-18}, and have applications in various domains, from robotics~\cite{my-hs-atarr-95} and assembly planning~\cite{hlw-gfapm-00} through Geographic
Information Systems (GIS)~\cite{DBLP:conf/gis/KreveldSW04} to protein structure determination~\cite{DBLP:journals/jcb/MartinYBZD11}, to mention just a few uses. The arrangements packages of \cgal{} have been developed since the early days of \cgal, first for planar arrangements and maps~\cite{DBLP:journals/jea/FlatoHHNE00,   DBLP:journals/comgeo/WeinFZH07}, Boolean operations, and Minkowski sums~\cite{bfhhm-epsph-15}. Then, envelopes of surfaces in three-dimensions have been added~\cite{m-rgece-06}. Finally, a major effort has been undertaken to supports two-dimensional arrangements on (not necessarily planar) surfaces~\cite{bfhks-apsca-10,bfhmw-apsgf-10}.

Given a surface $S$ in \Rthree{} and a set $\calC$ of curves embedded in this surface, the curves subdivide $S$ into cells of dimension~$0$ (vertices),~$1$ (edges), and~$2$ (faces). This subdivision is the arrangement $\calA(\calC)$ induced by $\calC$ on $S$~\cite{fhw-caass-12}. Arrangements embedded in curved surfaces in \Rthree{} are generalizations of arrangements embedded in the plane. The \iiDArrangementsPackage{} package~\cite{cgal:wfzh-a2-22}
can be used to construct, maintain, alter, and display 2D arrangements embedded in ruled curved surfaces, such as, spheres, ellipses, tori, cones, paraboloids, and the plane. It also supports queries on such arrangements, such as point location and vertical ray shooting. One of the main
components of the \iiDArrangementsPackage{} package is the \cppLstinline{Arrangement_2<Traits, Dcel>} class template. An instance of this template is used to represent an arrangement embedded
in the plane.  Table~\ref{tab:aos} lists the \cmake{} flags associated with the \iiDArrangementsPackage{} module.
% Currently, only instances of the
% \cppLstinline{Arrangement_2<Traits,Dcel>} class template are supported.
A description of the two template parameters of this class template follows.

%%%%%%%% Arrangement Module Flags
\begin{table}[!htp]
 \caption{\iiDArrangementsPackage{} module flags}
  \centering\begin{tikzpicture}
  \matrix (first) [tableModuleFlags,
    column 1/.style={nodes={text width=17.4em}},
    column 2/.style={nodes={text width=4.6em}},
    column 3/.style={nodes={text width=4.6em}},
    column 4/.style={nodes={text width=21.5em}},
    row 6/.style={nodes={minimum height=2.8em}}
  ] {
    Name & Type & Default & Description\\
    \cmakeLstinline{AOS2_GEOMETRY_TRAITS_NAME} & \cmakeLstinline{String} &       \myLstinline{segment} & The basic geometry traits\\
    \myLstinline{AOS2_EXTEND_VERTEX} & \cmakeLstinline{Boolean} & \myLstinline{false} & Determines whether to extend the vertex type\\
    \myLstinline{AOS2_EXTEND_HALFEDGE} & \cmakeLstinline{Boolean} & \myLstinline{false} & Determines whether to extend the halfedge type\\
    \myLstinline{AOS2_EXTEND_FACE} & \cmakeLstinline{Boolean} & \myLstinline{false} & Determines whether to extend the face type\\
    \myLstinline{AOS2_POINT_LOCATION_BINDINGS} & \cmakeLstinline{Boolean} &       \myLstinline{true} & Determines whether to generate bindings for point location and vertical ray shooting queries\\
  };
 \end{tikzpicture}
 \label{tab:aos}
\end{table}

\begin{itemize}
  \item The \cppLstinline{Traits} template-parameter determines the family of curves that induce the arrangement. The parameter should be substituted with a model of the basic arrangement traits concept or one or more concepts that refine the basic concept. A model of the basic traits concept defines the types of x-monotone curves and two-dimensional points and supports basic geometric predicates on them. A rather large directed acyclic graph is required to capture the entire hierarchy of the geometry traits-class concepts; therefore, we typically use subgraphs to describe the refinement relations among closely related concepts, and refer to these subgraph as clusters. Figure~\ref{fig:atc} depicts four clusters. The list of supported traits class templates follows. For each class template we describe the family of curves it handles.
  %
  \begin{compactenum}
  \item \cppLstinline{Arr_non_caching_segment_basic_traits_2<>}---handles segments.
  \item \cppLstinline{Arr_segment_traits_2<>}---handles segments, where each segment is represented a by its supporting line in addition to its two endpoints.
  \item \cppLstinline{Arr_linear_traits_2<>}---handles linear curves, i.e., segments, rays, and lines.
  \item \cppLstinline{Arr_polyline_traits_2<>}---handles polylines.
  \item \cppLstinline{Arr_circle_segment_traits_2<>}---handles segments and circular arcs.
  \item \cppLstinline{Arr_conic_traits_2<>}---handle conic arcs.
  \item \cppLstinline{Arr_rational_function_traits_2<>}---handle rational functions.
  \item \cppLstinline{Arr_Bezier_curve_traits_2<>}---handles B\'ezier curves of arbitrary degrees.
  \item \cppLstinline{Arr_algebraic_segment_traits_2<>}---handles algebraic curves of arbitrary degrees.
  \item \cppLstinline{Arr_polycurve_traits_2<>}---handle polycurves, which are
    piecewise curves that are not necessarily linear.
  \end{compactenum}

  The \cmake{} flag \cmakeLstinline{CGALPY_AOS2_GEOMETRY_TRAITS_NAME} specifies which geometry traits should be used for the generated bindings; see Table~\ref{tab:aos:gt}. Observe that instances of the class templates \cppLstinline{General_polygon_set_2<>} and \cppLstinline{Polygon_set_2<>} (see Section~\ref{ssec:modules:bso2}) employ 2D arrangement types. Bindings for instances of \cppLstinline{Polygon_set_2<>} and   \cppLstinline{General_polygon_set_2<>} are enabled as part of the bindings for the \iiDRegularizedBooleanSetOperationsPackage{} package. When bindings for the \iiDRegularizedBooleanSetOperationsPackage{} package are enabled, bindings of the \iiDArrangementsPackage{} package must be explicitly enabled as well. The traits type that substitutes the traits parameter determines the type of curves that bound the polygons or generalized polygons, and the type must be explicitly indicated too (unless the segment type is selected, which is the default). The traits type must also model the \cppLstinline{GeneralPolygonSetTraits_2} concept; see Figure~\ref{fig:atc:gps} for the relevant traits-concept cluster. The final traits type that is used for the bindings is automatically extended to satisfy this requirement. The details of this extension is given in Section~\ref{sec:extenders:arrTraits} of the appendix.
  %
\item The \cppLstinline{Dcel} template-parameter should be substituted with a type that models the \cppLstinline{ArrangementDcel} concept, which is used to represent the topological layout of the arrangement.\footnote{See     \url{https://doc.cgal.org/latest/Arrangement_on_surface_2/classArrangementDcel.html}.} This layout is, in particular, represented by a doubly-connected edge list data-structure (DCEL for short), which consists of containers of vertices, edges and faces and maintains the incidence   relations among these objects. We substitute this type with an instance of the template \cppLstinline{CGAL::Arr_dcel_base<V, H, F>}, where \cppLstinline{V}, \cppLstinline{H}, and
  \cppLstinline{F} are models of the concepts\linebreak
  \cppLstinline{ArrangementDcelVertex}, \cppLstinline{ArrangementDcelHalfedge}, and
  \cppLstinline{ArrangementDcelFace}, respectively; by default they are substituted with
  \cppLstinline{Arr_vertex_base<Traits::Point_2>},   \cppLstinline{Arr_halfedge_base<Traits::X_monotone_curve_2>}, and
  \cppLstinline{Arr_face_base}, respectively. In many applications it is necessary to extend the types of the DCEL main features. This is governed by three \cmake{} Boolean flags as follows. If any one of the \cmake{} variables \cmakeLstinline{CGALPY_AOS2_VERTEX_EXTENDED},
  \cmakeLstinline{CGALPY_AOS2_HALFEDGE_EXTENDED}, or   \cmakeLstinline{CGALPY_AOS2_FACE_EXTENDED} is set to true, the corresponding template parameter, \cppLstinline{V}, \cppLstinline{H}, or \cppLstinline{F}, is substituted with instances of \cppLstinline{Arr_extended_vertex<Vb, VertexData>},
  \cppLstinline{Arr_extended_halfedge<Hb, HalfedgeData>}, or
  \cppLstinline{Arr_extended_face<Fb, FaceData>}, respectively, where \cppLstinline{Vb}, \cppLstinline{Hb}, and \cppLstinline{Fb} are the basic types above. It is impossible to define a custom C++ type from Python code. Therefore, when the bindings are generated each one of the
  \cppLstinline{VertexData}, \cppLstinline{HalfedgeData}, and \cppLstinline{FaceData} template parameters must be substituted with a C++ type known at the time the bindings were   implemented. Flexibility is nevertheless retained by substituting every one of these parameters with the generic Python object \cppLstinline{py::object} when the respective cell is extended.\footnote{For more information on Python objects, see, e.g., \url{https://docs.python.org/3/library/functions.html?highlight=object\#object}.} This object provides a general interface to Python objects.
  %
  If bindings for the \iiDRegularizedBooleanSetOperationsPackage{} package is enabled, the template parameters \cppLstinline{H} and \cppLstinline{F} above are substituted with types that also model the concepts \cppLstinline{GeneralPolygonSetDcelHalfedge}, and \cppLstinline{GeneralPolygonSetDcelFace}, respectively; see Section~\ref{ssec:modules:bso2}. The final types that are used for the bindings are automatically extended to respect this requirement. The details of this extension is given in Section~\ref{sec:extenders:arrDcel} of the appendix.
\end{itemize}

\begin{figure}[!htp]
  \def\name#1{\scriptsize\cppLstinline{#1}}
  \tikzset{concept/.style={rectangle split,rectangle split parts=1,draw,
    fill=white,blur shadow,rounded corners,align=center}}
  \captionsetup[subfigure]{justification=centering}
  \centering%
  \subfloat[]{\label{fig:atc:central}
    \begin{forest}
      [\name{AosBasicTraits_2},for tree={concept,edge={-latex}}
        % forked edges
        [\name{AosXMonotoneTraits_2}
          [\name{AosTraits_2}]
        ]
      ]
    \end{forest}}\quad
  \subfloat[]{\label{fig:atc:landmark}
    \begin{forest}
      [\name{AosBasicTraits_2},name=abt,for tree={concept,edge={-latex}}
        % forked edges
        [\name{AosApproximateTraits_2}
          [,phantom]
          [\name{AosLandmarkTraits_2},name=alt,before drawing tree={x=0}]
        ]
        [\name{AosConstructXMonotoneCurveTraits_2},name=acxmt]
      ]
      \draw[-latex] (acxmt) to (alt);
      \end{forest}}\\
    %
  \subfloat[]{\label{fig:atc:openBoundary}
    \begin{forest}
      [\name{AosBasicTraits_2},name=abt,before drawing tree={x=0pt},for tree={concept,edge={-latex}}
        % forked edges
        [\name{AosVerticalSideTraits_2}
          [\name{AosLeftSideTraits_2}
            [\name{AosOpenLeftTraits_2},name=olt
              [,phantom]
              [\name{AosOpenBoundaryTraits_2},name=oyt,before drawing tree={x=0pt}]
            ]
          ]
          [\name{AosRightSideTraits_2}
            [\name{AosOpenRightTraits_2},name=ort]
          ]
        ]
        [\name{AosHorizontalSideTraits_2}
          [\name{AosBottomSideTraits_2}
            [\name{AosOpenBottomTraits_2},name=obt]
          ]
          [\name{AosTopSideTraits_2}
            [\name{AosOpenTopTraits_2},name=ott]
          ]
        ]
      ]
      \draw[-latex] (ort) to (oyt);
      \draw[-latex] (obt) to (oyt);
      \draw[-latex] (ott) to (oyt);
      \end{forest}}\\
    %
  \subfloat[]{\label{fig:atc:sphericalBoundary}
    \begin{forest}
      [\name{AosBasicTraits_2},name=abt,before drawing tree={x=0pt},for tree={concept,edge={-latex}}
        % forked edges
        [\name{AosVerticalSideTraits_2}
          [\name{AosLeftSideTraits_2}
            [,phantom]
            [\name{AosIdentifiedVerticalTraits_2},name=ivt
              [,phantom]
              [\name{AosSphericalBoundaryTraits_2},name=sbt,before drawing tree={x=0pt}]
            ]
          ]
          [\name{AosRightSideTraits_2},name=rst]
        ]
        [\name{AosHorizontalSideTraits_2}
          [\name{AosBottomSideTraits_2}
            [\name{AosContractedBottomCurveTraits_2},name=cbt]
          ]
          [\name{AosTopSideTraits_2}
            [\name{AosContractedTopCurveTraits_2},name=ctt]
          ]
        ]
      ]
      \draw[-latex] (cbt) to (sbt);
      \draw[-latex] (ctt) to (sbt);
      \draw[-latex] (rst) to (ivt);
      \end{forest}}
  \caption[]{%
    \subref{fig:atc:central}~The central cluster.%
    \subref{fig:atc:landmark}~The landmark cluster.%
    \subref{fig:atc:openBoundary}~The open boundary cluster.%
    \subref{fig:atc:sphericalBoundary}~The spherical boundary cluster.}
  \label{fig:atc}
\end{figure}

%%%%%%%% Arrangement Geometry Traits
\begin{table}[!htp]
  \caption{2D arrangement geometry traits options}
  \centering\begin{tikzpicture}
   \matrix (first) [tableName,
     column 1/.style={nodes={text width=18em}},
     column 2/.style={nodes={text width=31em}}
   ] {
     \cmakeLstinline{AOS2_GEOMETRY_TRAITS_NAME} & Type\\
     \myLstinline{nonCachingSegment} &
       \cppLstinline{Arr_non_caching_segment_basic_traits_2<Kernel>}\\
     \myLstinline{segment} & \cppLstinline{Arr_segment_traits_2<Kernel>}\\
     \myLstinline{linear} & \cppLstinline{Arr_linear_traits_2<Kernel>}\\
     \myLstinline{conic} &
       \cppLstinline{Arr_conic_traits_2<RatKernel, AlgKernel, NtTraits>}\\
     \myLstinline{circleSegment} &
       \cppLstinline{Arr_circle_segment_traits_2<Kernel>}\\
     \myLstinline{algebraic} &
       \cppLstinline{Arr_algebraic_segment_traits_2<Coefficient>}\\
   };
  \end{tikzpicture}
  \label{tab:aos:gt}
\end{table}

The code excerpt shown in Listing~\ref{lst:cmake:aos2EpecFaceExtended} in the \cmake{} language sets the \cmake{} flags for our next example shown in Listing~\ref{lst:py:aos2Fex}. This example constructs an arrangement with two faces. The arrangement is induced by line segments and its face type is extended. The properties of the bounded face and the unbounded face are initialized with Python integer objects '0' and '1', respectively.

\begin{lstfloat}
  \def\filename{aos2_epec_face_extended_release.cmake}%
  \lstinputlisting[style=cmakeFramedStyle, basicstyle=\normalsize,%
                   label={lst:cmake:aos2EpecFaceExtended},%
                   caption={\cmake{} flag settings used to generate bindings for 2D arrangements with their faces extended.}]%
                  {\cmakeDir\filename}
\end{lstfloat}

\begin{lstfloat}
  \def\filename{aos2_fex.py}%
  \lstinputlisting[style=pythonFramedStyle,basicstyle=\normalsize,
                   firstline=14,
                   label={lst:py:aos2Fex},
                   caption={Constructing an arrangement with its faces extended and initializing their data.}]
                  {\pythonDir\filename}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsection{2D Regularized Boolean Set Operation Bindings}
\label{ssec:modules:bso2}
% -----------------------------------------------------------------------------
The \cgal{} package \iiDRegularizedBooleanSetOperationsPackage{} consists of the implementation of regularized Boolean set-operations, intersection predicates, and point containment predicates on point sets bounded by weakly $x$-monotone curves in two-dimensional Euclidean space~\cite{cgal:fwzh-rbso2-22}. The \iiDRegularizedBooleanSetOperationsPackage{} module is not associated with \cmake{} flags (besides the flag \cmakeLstinline{CGALPY_BOOLEAN_SET_OPERATIONS_2_BINDINGS}, which indicates whether to generate bindings for this module). The Boolean set operations supported by this package depend on the
\iiDArrangementsPackage{} package. If the operations are applied on (linear) polygons they also depend on the \iiDPolygonsPackage{} package. Recall, that both further depend on the
\iiDandiiiDGeometryKernelPackage{} package. Therefore, bindings for these packages must be explicitly enabled as well when bindings for the \iiDRegularizedBooleanSetOperationsPackage{} package are enabled.

The code excerpt shown in Listing~\ref{lst:cmake:bso2EpecCs} in the \cmake{} language sets the \cmake{} flags for our next example. Applying these settings followed by the native build commands generates a library, the basename of which is \myLstinline{CGALPY_kerEpec_ aos2Cs_bso2_pol2}. It supports bindings for the types below and operations on these types, but nothing else.
\begin{compactitem}
\item kernel types,
\item line segment and circular arc,
\item arrangement in the plane induced by curves of the above types,
\item generalized polygon and generalized polygon with holes bounded by curves of the above types, and
\item Boolean operations on generalized polygons of the above types.
\end{compactitem}

\begin{lstfloat}
  \def\filename{bso2_epec_cs_release.cmake}%
  \lstinputlisting[style=cmakeFramedStyle, basicstyle=\normalsize,%
                   label={lst:cmake:bso2EpecCs},%
                   caption={\cmake{} flag settings used to generate bindings for 2D regularized Boolean operations on generalized polygons bounded by line segments and circular arcs.}]%
                  {\cmakeDir\filename}
\end{lstfloat}

This library can be used to execute the Python example shown in Listing~\ref{lst:py:circleSegmentPolygons}; the example constructs a general polygon-set that represents the point set depicted in Figure~\ref{fig:csp}. It is the result of the union of four disjoint circles and four rectangles. Each circle is represented as a generalized polygon bounded by two x-monotone circular arcs. The union is computed incrementally, resulting with a single generalized polygon with a single hole. Note that as the four circles are disjoint, their
union is computed with the \cppLstinline{insert()} function, while the union with the rectangles is computed with the \cppLstinline{join()} function.

\begin{lstfloat}
  \def\filename{Boolean_set_operations_2/circle_segment.py}%
  \lstinputlisting[style=pythonFramedStyle, basicstyle=\normalsize,%
                   firstline=15,lastline=55,%
                   label={lst:py:circleSegmentPolygons},%
                   caption={Constructing a general polygon-set that represents the point set depicted in Figure~\ref{fig:csp}.}]%
                  {\pythonDir\filename}
\end{lstfloat}

\begin{figure}[!htp]
  \def\name#1{\scriptsize\cppLstinline{#1}}
  \tikzset{concept/.style={rectangle split,rectangle split parts=1,draw,
      fill=white,blur shadow,rounded corners,align=center}}
  \captionsetup[subfigure]{justification=centering}
  \centering%
  \subfloat[]{\label{fig:csp}
    \begin{tikzpicture}
    \fill[lightgray] (0.5,0) rectangle (2.5,1);
    \fill[lightgray] (0.5,2) rectangle (2.5,3);
    \fill[lightgray] (0,0.5) rectangle (1,2.5);
    \fill[lightgray] (2,0.5) rectangle (3,2.5);
    \filldraw[fill=gray,draw=black](0.5,0.5) circle (0.5);
    \filldraw[fill=gray,draw=black](2.5,0.5) circle (0.5);
    \filldraw[fill=gray,draw=black](0.5,2.5) circle (0.5);
    \filldraw[fill=gray,draw=black](2.5,2.5) circle (0.5);
    \draw[black] (0.5,0) rectangle (2.5,1);
    \draw[black] (0.5,2) rectangle (2.5,3);
    \draw[black] (0,0.5) rectangle (1,2.5);
    \draw[black] (2,0.5) rectangle (3,2.5);
    \end{tikzpicture}}\quad
  \subfloat[]{\label{fig:atc:gps}
    \begin{forest}
      [\name{AosXMonotoneTraits_2},for tree={concept,edge={-latex}}
        % forked edges
        [\name{AosDirectionalXMonotoneTraits_2}
          [\name{GeneralPolygonSetTraits_2}]
        ]
      ]
    \end{forest}}
  \caption[]{%
    \subref{fig:csp}~A generalized polygon with holes bounded by circular
      arcs and line segments.
    \subref{fig:atc:gps}~The general point-set cluster of concepts.}
  \label{fig:bso2}
\end{figure}

An arrangement data structure is internally used to represent the point set maintained by a general polygon-set object; it is possible to obtain it and apply further operations on it, as demonstrated by the code excerpt shown in Listing~\ref{lst:py:circleSegmentPolygonsArr}.

\begin{lstfloat}
  \def\filename{Boolean_set_operations_2/circle_segment.py}%
  \lstinputlisting[style=pythonFramedStyle, basicstyle=\normalsize,%
                   firstline=56,%
                   label={lst:py:circleSegmentPolygonsArr},%
                   caption={Extracting the arrangement from a point set.}]%
                  {\pythonDir\filename}
\end{lstfloat}

The bindings for the \iiDArrangementsPackage{} package includes bindings for the geometry traits and the DCEL suitable for Boolean operations. In particular, the traits must model the concept \cppLstinline{GeneralPolygonSetTraits_2}; see Figure~\ref{fig:atc:gps}.

% -----------------------------------------------------------------------------
\subsection{2D Minkowski Sums}
\label{ssec:modules:ms2}
% -----------------------------------------------------------------------------
Given two sets of points $\calA, \calB \in \Rd$ their Minkowski sum, denoted by $\calA \oplus \calB$, is their point-wise sum, namely the set $\{a+b|\, a \in \calA,b \in \calB\}$. The \cgal{} package \iiDMinkowskiSumsPackage{} contains functions that compute the planar Minkowski sum of two polygons and the planar Minkowski sum of a simple polygon and a disc---an operation also referred to as offsetting or dilating a polygon. The package also supports inner offsetting a polygon (also referred to as insetting), which is equivalent to the complement of the offset of (i) a disk and (ii) the complement of a polygon~\cite{cgal:w-rms2-22}. The \iiDMinkowskiSumsPackage{} module is not associated with any \cmake{} flags (besides the flag \lstinline[language={Cmake}]{CGALPY_MINKOWSKI_SUM_2_BINDINGS}, which indicates whether to generate bindings for this module). Similar to the case of generating bindings of Boolean operations on (linear) polygons supported by the \iiDRegularizedBooleanSetOperationsPackage{} package, the operations supported by this package depend on the \iiDandiiiDGeometryKernelPackage{}, \iiDArrangementsPackage{}, and
\iiDPolygonsPackage{} packages. Therefore, bindings for these packages must be explicitly enabled as well when bindings for the \iiDMinkowskiSumsPackage{} package are enabled.  The result of the inset and offset operations is a generalized polygon bounded by line
segments and circular arc. Binding for a type that represents such polygons, that is, an instance of \cppLstinline{CGAL::General_polygon_with_holes_2<>} is generated as well.

The function \cppLstinline{CGAL::minkowski_sum()} is extremely overloaded. It can be used to compute the Minkowski sum of two polygons either applying the \emph{convex-decomposition} approach or the \emph{reduced-convolution} approach. When applying the \emph{convex-decomposition} approach we first decompose each summand
into convex sub-polygons. The function template \cppLstinline{CGAL::minkowski_sum_by_full_convolution_2()} applies a third approach, namely \emph{full convolution}. For more information on the various approaches refer to the manual.

There are two overloaded function templates \cppLstinline{CGAL::minkowski_sum()} that apply the \emph{reduced-convolution} approach; both accepts the two input polygons as input; one also accepts a specific geometry traits as input (while the other constructs and uses a default traits object). Each type of the summands must represent either a simple polygon or a polygon with holes. The signature of the former is shown in Listing~\ref{lst:cpp:minkSum}, where each of \cppLstinline{PolygonType1} and \cppLstinline{PolygonType2} can be substituted either with an instance of \cppLstinline{Polygon_2<Kernel, Container>} or with and instance of \cppLstinline{Polygon_with_holes_2<Kernel, Container>}.
%
Thus, given a specific kernel and container types, we get eight overloaded instances that apply the \emph{reduced-convolution} approach in total. (The Container type determines the representation of the polygon's extreme points in memory.)

\begin{lstfloat}
  \begin{lstlisting}[style=cppFramedStyle,basicstyle=\normalsize,
                     label={lst:cpp:minkSum},
                     caption={The signature of one of the \cppLstinline{CGAL::minkowski_sum_2} overloaded function templates.}]
template <typename Kernel, typename Container>
Polygon_with_holes_2<Kernel, Container>
minkowski_sum_2(const PolygonType1<Kernel, Container>& p,
                const PolygonType2<Kernel, Container>& q)
\end{lstlisting}
\end{lstfloat}

There are two sets of function templates \cppLstinline{CGAL::minkowski_sum()} that apply the \emph{convex-decomposition} approach; all functions accepts two polygons as input; functions in one set also accept a specific geometry traits as input. As with the functions that apply the \emph{reduced-convolution} approach, each type of the summands must be substituted either with a type that represents a simple polygon or a type that represents a polygon with holes. Each set consists of two function templates; one is parameterized with the type that represents a single decomposition strategy that should be applied to both summands and another one that is parameterized with two types that
represent two decomposition strategies that should be applied to the two summands, respectively. The package provides four types of decomposition strategies; however, only two can be applied to a polygon with holes. Listing~\ref{lst:minkSumConvexDecomposition} shows the signatures of the two function templates that do not accept a traits parameter.
%
We get 10~overloaded instances of functions that apply the \emph{convex-decomposition} approach, do not accept a traits parameter, and are parameterized with a single decomposition strategy. We get 36~overloaded instances of functions that apply the
\emph{convex-decomposition} approach, do not accept a traits parameter, and are parameterized with two decomposition strategies. Thus, given a specific kernel and container types, we get $2 \times (10 + 36) = 92$ overloaded instances of functions that apply the \emph{convex-decomposition} approach.

The \cppLstinline{approximated_inset_2(P, r, eps, oi)} function template accepts a polygon $P$, an inset radius $r$, (a floating-point number\index{number!floating-point}) $\epsilon > 0$, and an output iterator\index{iterator!output} \cppLstinline{oi}; dereferencing the iterator must yield an instance of the class template
\cppLstinline{CGAL::Gps_circle_segment_traits_2<Kernel>::Polygon_2}. It constructs an approximation of the inset of $P$ by the radius $r$, where the approximation error is bounded by $\epsilon$. The function returns the polygons that approximate the inset polygon through the output iterator \cppLstinline{oi}.

The code excerpt shown in Listing~\ref{lst:py:approxInset} demonstrates the construction of an approximated inner offset; see Figure~\ref{fig:ms2:inset}.

\begin{lstfloat}
  \def\filename{approx_inset.py}%
  \lstinputlisting[style=pythonFramedStyle, basicstyle=\normalsize,%
                   firstline=35,%
                   label={lst:py:approxInset},%
                   caption={Computing the approximated inner offset.}]%
                  {\pythonDir\filename}
\end{lstfloat}

\begin{SCfigure}[][!t]
 \begin{tikzpicture}[scale=0.4]
    \coordinate (c1) at (8,3);
    \coordinate (p11) at (8.94868,3.31623);
    \coordinate (p12) at (7.05132,3.31623);
    %
    \coordinate (c2) at (6,7);
    \coordinate (p21) at (6.78087,6.3753);
    \coordinate (p22) at (7,7);      %\draw (6,9) circle (3pt);
    %
    \filldraw [color=polyADarkColor,fill=polyALightColor,thick]
      (4, 0)--(7,0)--(8,3)--(9,0)--(13,0)--(13,8)--(7,8)--(7,9)--
      (13,9)--(13,14)--(0,14)--(0,12)--(6,9)--(6,7)--(2,2)--cycle;
    \filldraw [color=polyCDarkColor,fill=polyCLightColor,thick]
      let \p1 = ($(p11) - (c1)$),
        \p2 = ($(p12) - (c1)$),
        \n0 = {veclen(\x1,\y1)}, % radius
        \n1 = {atan2(\y1,\x1)},  % initial angle
        \n2 = {atan2(\y2,\x2)},  % Final angle
        \p3 = ($(p21) - (c2)$),
        \p4 = ($(p22) - (c2)$),
        \n3 = {veclen(\x3,\y4)}, % radius
        \n4 = {atan2(\y3,\x4)},  % initial angle
        \n5 = {atan2(\y3,\x4)}   % Final angle
      in
        (7,7)--(12,7)--(12,1)--(9.72076,1)--(9.29057,2.29057)--(p11)arc(\n1:\n2:\n0)--
        (6.3932,1.34189)--(6.27924,1)--(4.41421,1)--(3.34,2.07422)--(3.53148,2.31357)--
        (p21)arc(\n4:\n5:\n3)--cycle;
    \filldraw [color=polyCDarkColor,fill=polyCLightColor,thick]
      (1,13)--(12,13)--(12,10)--(7,10)--
      (6.5,9.86603)--
      (6.44721,9.89443)--(4.78885,10.7236)--(1,12.618)--(1,13)--cycle;
      %\draw (7,9) circle (3pt);
      %\draw (6,9) circle (3pt);
  \end{tikzpicture}
  \caption{%
    The inset (yellow) of a polygon (blue) with a tight corridor consists of two generalized polygons bounded by line segments and circular arcs.}
  \label{fig:ms2:inset}
\end{SCfigure}

% -----------------------------------------------------------------------------
\subsection{2D Triangulation Bindings}
\label{ssec:modules:tri2}
% -----------------------------------------------------------------------------
Triangulation is perhaps the most common term in the lexicon of computational geometry. Triangulations are ubiquitous geometric data structures, which are used in numerous areas, such as, GIS, robotics, geometric modeling and meshing to name a few; see, e.g.,~\cite{by-ag-98} for a survey on triangulations. The triangulation packages of \cgal{} are integral parts of the library and have constantly improved and enhanced
since the early days of \cgal{}. In two-dimensions \cgal{} offers basic, Delaunay and regular triangulations, as well as constrained triangulations and constrained Delaunay triangulations. In three dimensions \cgal{} offers basic, Delaunay, and regular triangulations. \cgal{} also offers periodic triangulations both in the plane and in space~\cite{ct-cpt-09}.

A triangulation of a set of points $\calP$ in \Rtwo is a partition of the convex hull of $\calP$ into triangles whose vertices are the points of $\calP$. Together with the unbounded face having the convex hull boundary as its frontier, the triangulation forms a partition of \Rtwo. Any two facets (2-face) are either disjoint or share a common
edge (1-face) or vertex (0-face). A triangulation can be described as a simplicial complex. The binding module \iiDTriangulationsPackage{} consists of bindings of types provided by the \cgal{} packages \iiDTriangulationsPackage{} and \iiDPeriodicTriangulationsPackage{}. Table~\ref{tab:tri2} lists the \cmake{} flags associated with the \iiDTriangulationsPackage{} module.

%%%%%%%% 2D Triangulation Module Flags
\begin{table}[!htp]
  \caption{\iiDTriangulationsPackage{} module flags.}
  \centering\begin{tikzpicture}
  \matrix (first) [tableModuleFlags,
    column 1/.style={nodes={text width=16.0em}},
    column 3/.style={nodes={text width=5.7em}},
    column 4/.style={nodes={text width=21.6em}},
    row 6/.append style={nodes={minimum height=2.8em}}
  ] {
    Name & Type & Default & Description\\
    \cmakeLstinline{TRI2_NAME} & String & \myLstinline{plain} &
      The 2D triangulation type\\
    \cmakeLstinline{TRI2_VERTEX_WITH_INFO}      & Boolean & \myLstinline{false} & Determines whether the vertex type is extended\\
    \cmakeLstinline{TRI2_FACE_WITH_INFO}        & Boolean & \myLstinline{false} & Determines whether the face type is extended\\
    \cmakeLstinline{TRI2_INTERSECTION_TAG_NAME} & String  & \myLstinline{ncirc} & The intersection tag\\
    \cmakeLstinline{TRI2_HIERARCHY}               & Boolean & \myLstinline{false} & Determines whether to generate the binding for a hierarchy triangulation\\
  };
  \end{tikzpicture}
  \label{tab:tri2}
\end{table}

The \iiDTriangulationsPackage{} package~\cite{cgal:y-t2-22} provides several class templates, instances of which can be used to represent a variety of 2D triangulations. In particular, the package provides the following class templates:
\begin{compactenum}
\item \cppLstinline{Triangulation_2<Traits, Tds>},
\item \cppLstinline{Regular_triangulation_2<Traits, Tds>},
\item \cppLstinline{Delaunay_triangulation_2<Traits, Tds>},
\item \cppLstinline{Constrained_triangulation_2<Traits, Tds, Itag>},
\item \cppLstinline{Constrained_Delaunay_triangulation_2<Traits, Tds, Itag>}, and
\item \cppLstinline{Triangulation_hierarchy_2<Triangulation_2>}
\end{compactenum}
Instances of the \cppLstinline{Delaunay_triangulation_2<>} and \cppLstinline{Regular_triangulation_2<>} class templates can be used to represent Delaunay and regular triangulation, respectively. In a regular triangulation points have an associated weight, and some points can be hidden and do not result in vertices of the
triangulation. The class template \cppLstinline{Triangulation_hierarchy_2} enables fast point location queries. When instantiated its template parameter must be substituted
with an instance of any other triangulation class template.

The \iiDPeriodicTriangulationsPackage{} package~\cite{cgal:k-pt2-13-22} supports triangulations of sets of points in the two-dimensional flat torus~\cite{ct-cpt-09}. This
package provides the class templates
\begin{compactenum}
\item \cppLstinline{Periodic_2_triangulation_2<Traits, Tds>},
\item \cppLstinline{Periodic_2_Delaunay_triangulation_2<Traits, Tds>}, and
\item \cppLstinline{Periodic_2_triangulation_hierarchy_2<PeriodicTriangulation>}
\end{compactenum}

The \cmake{} flag \cmakeLstinline{CGALPY_TRI2_NAME} specifies the particular type of triangulation, bindings for which should be generated; see Table~\ref{tab:tri2:names}.

\begin{table}[!htp]
  \caption{2D triangulation name options}
  \centering\begin{tikzpicture}
  \matrix (first) [tableName,
    column 1/.style={nodes={text width=11.5em}},
    column 2/.style={nodes={text width=37.5em}}
  ] {
    \cmakeLstinline{TRI2_NAME} & Type\\
    \myLstinline{plain} & \cppLstinline{Triangulation_2<Traits, Tds>}\\
    \myLstinline{regular} & \cppLstinline{Regular_triangulation_2<Traits, Tds>}\\
    \myLstinline{delaunay} & \cppLstinline{Delaunay_triangulation_2<Traits, Tds>}\\
    \myLstinline{constrained} & \cppLstinline{Constrained_triangulation_2<Traits, Tds, Itag>}\\
    \myLstinline{constrainedDelaunay} & \cppLstinline{Constrained_Delaunay_triangulation_2<Traits, Tds, Itag>}\\
    \myLstinline{periodicPlain} & \cppLstinline{Periodic_2_triangulation_2<Traits, Tds>}\\
    \myLstinline{periodicDelaunay} & \cppLstinline{Periodic_2_Delaunay_triangulation_2<Traits, Tds>}\\
  };
  \end{tikzpicture}
  \label{tab:tri2:names}
\end{table}

%% \cppLstinline{TriangulationTraits_2}
%% \cppLstinline{RegularTriangulationTraits_2}
%% \cppLstinline{DelaunayTriangulationTraits_2}
%% \cppLstinline{ConstrainedTriangulationTraits_2}
%% \cppLstinline{ConstrainedDelaunayTriangulationTraits_2}
%% \cppLstinline{AlphaShapeTraits_2}
%% \cppLstinline{WeightedAlphaShapeTraits_2}
%% \cppLstinline{Periodic_2TriangulationTraits_2}
%% \cppLstinline{Periodic_2DelaunayTriangulationTraits_2}
%% \cppLstinline{Periodic_3AlphaShapeTraits_2}
When any template above is instantiated the template parameter \cppLstinline{Traits} must be substituted with a model of a suitable geometric traits concept; this model is referred to as the geometric traits class; it provides the type of points to use as well as elementary operations on points of the indicated type. The type of traits used for the generated bindings is determined based on the selection of the triangulation type as explained below. It is conveniently defined in C++ as \cppLstinline{Dt::Geom_traits}, where \cppLstinline{Dt} is a triangulation instance. This type is exposed as a Python attribute with the same name under \pyLstinline{Triangulation_2} (which in turn is nested under the Python namespace \pyLstinline{Tri2}). Figure~\ref{tab:tri2:concept-hierarchy} depicts the 2D triangulation traits concept hierarchy. Any kernel instance is a model of any non-periodic traits concept; thus, when one of the templates
\begin{compactenum}
\item \cppLstinline{Triangulation_2<Traits, Tds>},
\item \cppLstinline{Regular_triangulation_2<Traits, Tds>},
\item \cppLstinline{Delaunay_triangulation_2<Traits, Tds>},
\item \cppLstinline{Constrained_triangulation_2<Traits, Tds, Itag>}, or
\item \cppLstinline{Constrained_Delaunay_triangulation_2<Traits, Tds, Itag>}
\end{compactenum}
is instantiated, the \cppLstinline{Traits} parameter is substituted with the \cppLstinline{Kernel} type (the selected kernel; see Section~\ref{ssec:modules:kernel}). When one of the templates
\begin{compactenum}
\item \cppLstinline{Periodic_2_triangulation_2<Traits, Tds>} or
\item \cppLstinline{Periodic_2_Delaunay_triangulation_2<Traits, Tds>}
\end{compactenum}
is instantiated, the \cppLstinline{Traits} parameter is substituted with \cppLstinline{Periodic_2_triangulation_traits_2<Kernel>} or \cppLstinline{Periodic_2_Delaunay_triangulation_traits_2<Kernel>}, respectively.
%
Observe that when a Delaunay triangulation instance is used to define an alpha shape type (see Section~\ref{ssec:modules:as2}), the traits parameter must be substituted with a traits class that models the \cppLstinline{AlphaShapeTraits_2} concept. Similarly, when a regular triangulation instance is used to define a fixed alpha shape type (see Section~\ref{ssec:modules:as2}), the traits parameter must be substituted with a traits class that models the \cppLstinline{WeightedAlphaShapeTraits_2} concept. Also in these
cases the selected kernel serves as the traits.

\begin{figure}[!htp]
  \def\name#1{\scriptsize\cppLstinline{#1}}
  \tikzset{%
    concept/.style={rectangle,rounded corners,align=center,
      draw,fill=white,blur shadow,% drop shadow%
    }
  }
  \forestset{
    my tree style/.style={
      for tree={concept,
        parent anchor=south,
        child anchor=north,
        edge={->,>=stealth,black,thick},
        edge path={% |-| style branches from parent to child
          \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor)--(.child anchor)\forestoption{edge label};
        },
        if n children=3{% if a node has 3 children
          for children={% align the middle child with its parent
            if n=2{calign with current}{}
          }
        }{},
      }
    }
  }
  \centering%
  \begin{forest}
    my tree style
    [ \name{TriTr2}
      [ \name{RegularTriTr2}
        [ \name{WeightedAlphaShapeTr2} ]
      ]
      [ \name{Pr2TriTr2},name=p ]
      [ \name{DelaunayTriTr2},name=d
        [ \name{Pr2DelaunayTriTr2},name=pd
	  [ \name{Pr2AlphaShapeTr2} ]
        ]
        [ \name{AlphaShapeTr2} ]
      ]
      [ \name{ConstrainedTriTr2}
        [ \name{ConstrainedDelaunayTriTr2},name=cd ]
      ]
    ]
    \draw[->,>=stealth] (d.parent anchor)--(cd.child anchor);
    \draw[->,>=stealth] (p.parent anchor)--(pd.child anchor);
  \end{forest}
  \caption{The 2D triangulation traits concept hierarchy.
    \cppLstinline{Triangulation}, \cppLstinline{Periodic_2} and
    \cppLstinline{Traits_2} are abbreviated as \cppLstinline{Tri},
    \cppLstinline{Pr2}, and \cppLstinline{Tr2},
    respectively.}
  \label{tab:tri2:concept-hierarchy}
\end{figure}

The \cmake{} Boolean flag \cmakeLstinline{CGALPY_TRI2_HIERARCHY} indicates whether the type of triangulation, bindings for which should be generated, is an instance of one of the triangulation hierarchy templates, namely,
\begin{compactitem}
\item \cppLstinline{Triangulation_hierarchy_2<Triangulation_2>} and
\item \cppLstinline{Periodic_triangulation_hierarchy_2<PeriodicTriangulation_2>}.
\end{compactitem}
The template parameter in both cases is substituted with the triangulation selected via the \cmake{} flag \cmakeLstinline{CGALPY_TRI2_ NAME}, which also determines whether to use the non-periodic or periodic version above.

The type that substitutes the \cppLstinline{Tds} parameter models the concept \cppLstinline{TriangulationDataStructure_2}. An object of this type stores the combinatorial structure of the triangulation; it is an instance of the class template
\cppLstinline{Triangulation_data_structure_2<V, F>}. The types that substitute the \cppLstinline{V} and \cppLstinline{F} template parameters when the template
\cppLstinline{Triangulation_data_structure_2<V, F>} is instantiated represent the type of the vertex and the type of the face of the triangulation, respectively; they must model the concepts \cppLstinline{TriangulationDSVertexBase_2} and \cppLstinline{TriangulationDSFaceBase_2}, respectively. If the binding is generated for a periodic triangulation, these parameters must be substituted with types that also model the concepts \cppLstinline{Periodic_2TriangulationDSVertexBase_ 2} and
\cppLstinline{Periodic_2TriangulationDSFaceBase_2}, respectively. If the triangulation is used to define an alpha shape type, these parameters must be substituted with types that also model the concepts \cppLstinline{AlphaShapeVertex_2} and \cppLstinline{AlphaShapeFace_2}, respectively; see Section~\ref{ssec:modules:as2}. Finally, if the binding is generated for a hierarchy triangulation, e.g., an instance of the template parameter \cppLstinline{Triangulation_hierarchy_2<Triangulation_2>},
the \cppLstinline{V} template parameter must be substituted with a model of the concept
\cppLstinline{TriangulationHierarchyVertexBase_2}. (Observe that there is no special requirements on the type that substitutes the \cppLstinline{F} parameter in this case.) Similar to the 2D arrangement data structure, it is possible to extend the vertex and
face types of the triangulation. This is governed by two \cmake{} Boolean flags as follows. If any one of the \cmake{} variables \cmakeLstinline{CGALPY_TRI2_VERTEX_WITH_INFO} or
\cmakeLstinline{CGALPY_TRI2_FACE_WITH_INFO} is set to true, the corresponding template parameter, \cppLstinline{V} or \cppLstinline{F}, is substituted with instances of
\cppLstinline{CGAL::Triangulation_vertex_base_with_info_2<py::object, Traits, Vb>} or \cppLstinline{CGAL::Triangulation_face_base_with_info_2<py::object, Traits, Vb>},
respectively, where \cppLstinline{Vb} and \cppLstinline{Fb} are types that model the concepts above. The final vertex type is selected accordingly; it is explained in details in Section~\ref{sec:extenders:iitri} of the appendix.

The final vertex type is conveniently defined in C++ as \cppLstinline{Dt::Vertex}, where \cppLstinline{Dt} is the triangulation instance. This type is exposed as a Python attribute with the same name under \pyLstinline{Triangulation_2}.
%
The final face type is conveniently defined in C++ as \cppLstinline{Dt::Face}, where \cppLstinline{Dt} is the triangulation instance. This type is also exposed as a Python attribute with the same name under \pyLstinline{Triangulation_2}.

% -----------------------------------------------------------------------------
\subsection{2D Alpha Shape Bindings}
\label{ssec:modules:as2}
% -----------------------------------------------------------------------------
The alpha shape (a.k.a.\ alpha complex) of a set of points is one of
several notions of a shape formed by the set. Given a set of points
sampled in a 2D body, an alpha shape is demarcated by a frontier,
which is a linear approximation of the original boundary of the
body. A two-dimensional alpha shape object maintains an underlying
triangulation of a set of input points in the plane. There are two
distinguished versions of alpha shapes as follows. Basic alpha shapes
are based on the Delaunay triangulation and weighted alpha shapes are
based on its generalization, the regular triangulation, where the
euclidean distance is replaced by the power to weighted points.  The
package \iiDAlphaShapesPackage{}~\cite{cgal:d-as2-22} provides the
class template \cppLstinline{Alpha_shape_2<Dt,
  ExactAlphaComparisonTag>}. In a 2D alpha shape object represented by
an instance of this class template each $k$-simplex of the underlying
triangulation is associated with an interval that specifies for which
values of $\alpha$ the $k$-simplex belongs to the alpha shape.
Table~\ref{tab:as2} lists the \cmake{} flags associated with the
\iiDAlphaShapesPackage{} module.

%%%%%%%% 2D Alpha Shape Module flags
\begin{table}[!htp]
  \caption{\iiDAlphaShapesPackage{} module flags}
  \centering\begin{tikzpicture}
  \matrix (first) [tableModuleFlags,
    column 1/.style={nodes={text width=16em}},
    column 3/.style={nodes={text width=5.7em}},
    column 4/.style={nodes={text width=21.6em}}
  ] {
    Name & Type &  Default & Description\\
    \myLstinline{AS2_EXACT_COMPARISON} & Boolean & \myLstinline{false} &
      Determines whether to apply exact comparisons\\
  };
 \end{tikzpicture}
 \label{tab:as2}
\end{table}

% -----------------------------------------------------------------------------
\subsection{3D Triangulation Bindings}
\label{ssec:modules:tri3}
% -----------------------------------------------------------------------------
A triangulation of a set of points $\calP$ in \Rthree is a partition
of the convex hull of $\calP$ into tetrahedra whose vertices are the
points of $\calP$. Similar to the two-dimensional triangulation,
together with the unbounded cell having the convex hull boundary as
its frontier, the triangulation forms a partition of \Rthree. Any two
cells (3-face) are either disjoint or share a common facet (2-face),
edge (1-face) or vertex (0-face).  The binding module
\iiiDTriangulationsPackage{} consists of bindings of types provided by
the \cgal{} packages \iiiDTriangulationsPackage{} and
\iiiDPeriodicTriangulationsPackage{}. Table~\ref{tab:tri3} lists the
\cmake{} flags associated with the \iiiDTriangulationsPackage{}
module.

%%%%%%%% 3D Triangulation Module Flags
\begin{table}[!htp]
  \caption{\iiiDTriangulationsPackage{} module flags.}
  \centering\begin{tikzpicture}
  \matrix (first) [tableModuleFlags,
    row 5/.append style={nodes={minimum height=2.8em}}
  ] {
    Name & Type & Default & Description\\
    \cmakeLstinline{TRI3_NAME}                   & String & \myLstinline{plain}    & The 3D triangulation type\\
    \cmakeLstinline{TRI3_CONCURRENCY_NAME}      & String & \myLstinline{sequential} & The concurrency method\\
    \cmakeLstinline{TRI3_LOCATION_POLICY_NAME} & String & \myLstinline{compact}    & The location policy\\
    \cmakeLstinline{TRI3_HIERARCHY}             & Boolean & \myLstinline{false} & Determines whether to generate the binding for a hierarchy triangulation\\
  };
  \end{tikzpicture}
  \label{tab:tri3}
\end{table}

The \iiiDTriangulationsPackage{} package~\cite{cgal:pt-t3-22}
provides several class templates, instances of which can be used to
represent a variety 3D triangulations. In particular, the package
provides the following class templates:
\begin{compactenum}
\item \cppLstinline{Triangulation_3<Traits, Tds, Slds>},
\item \cppLstinline{Regular_triangulation_3<Traits, Tds, Slds>}, and
\item \cppLstinline{Delaunay_triangulation_3<Traits, Tds, LocationPolicy, Slds>}
\item \cppLstinline{Triangulation_hierarchy_3<Triangulation_3>}
\end{compactenum}
Instance of the \cppLstinline{Delaunay_triangulation_3<>} and
\cppLstinline{Regular_triangulation_3<>} class templates can be used
to represent Delaunay and regular triangulation, respectively. In a
regular triangulation points have an associated weight, and some
points can be hidden and do not result in vertices in the
triangulation. The template \cppLstinline{Triangulation_hierarchy_3} enables fast
point location queries. When instantiated its template parameter must
be substituted with an instance of any other triangulation class template.

The \iiiDPeriodicTriangulationsPackage{}
package~\cite{cgal:ct-pt3-22} supports triangulations of sets of
points in the three-dimensional flat torus~\cite{ct-cpt-09}. This
package provides the class templates
\begin{compactenum}
\item \cppLstinline{Periodic_3_triangulation_3<Traits, Tds>},
\item \cppLstinline{Periodic_3_regular_triangulation_3<Traits, Tds>}, and
\item \cppLstinline{Periodic_3_Delaunay_triangulation_3<Traits, Tds>}
\item \cppLstinline{Periodic_3_triangulation_hierarchy_3<PeriodicTriangulation>}
\end{compactenum}

The \cmake{} flag \myLstinline{CGALPY_TRI3_NAME} specifies the particular
types of triangulation, bindings for which should be generated; see
Table~\ref{tab:tri3:names}.

\begin{table}[!htp]
  \caption{3D triangulation name options}
  \centering\begin{tikzpicture}
  \matrix (first) [tableName,
    column 1/.style={nodes={text width=10em}},
    column 2/.style={nodes={text width=39em}}
  ] {
    \myLstinline{TRI3_NAME} & Type\\
    \myLstinline{plain} & \cppLstinline{Triangulation_3<Traits, Tds, Slds>}\\
    \myLstinline{regular} & \cppLstinline{Regular_triangulation_3<Traits, Tds, Slds>}\\
    \myLstinline{delaunay} & \cppLstinline{Delaunay_triangulation_3<Traits, Tds, LocationPolicy, Slds>}\\
    \myLstinline{periodicPlain} & \cppLstinline{Periodic_3_triangulation_3<Traits, Tds>}\\
    \myLstinline{periodicRegular} & \cppLstinline{Periodic_3_regular_triangulation_3<Traits, Tds>}\\
    \myLstinline{periodicDelaunay} & \cppLstinline{Periodic_3_Delaunay_triangulation_3<Traits, Tds>}\\
  };
  \end{tikzpicture}
  \label{tab:tri3:names}
\end{table}

%% \cppLstinline{TriangulationTraits_3}
%% \cppLstinline{RegularTriangulationTraits_3}
%% \cppLstinline{DelaunayTriangulationTraits_3}
%% \cppLstinline{AlphaShapeTraits_3}
%% \cppLstinline{FixedAlphaShapeTraits_3}
%% \cppLstinline{WeightedAlphaShapeTraits_3}
%% \cppLstinline{FixedWeightedAlphaShapeTraits_3}
%% \cppLstinline{Periodic_3TriangulationTraits_3}
%% \cppLstinline{Periodic_3RegularTriangulationTraits_3}
%% \cppLstinline{Periodic_3DelaunayTriangulationTraits_3}
%% \cppLstinline{Periodic_3AlphaShapeTraits_3}
When any template above is instantiated the template parameter
\cppLstinline{Traits} must be substituted with a model of a suitable
geometric traits concept; this model is referred to as the geometric
traits class; it provides the type of points to use as well as
elementary operations on points of the indicated types. The type of
traits used for the generated bindings is determined based on the
selection of the triangulation type as explained below. It is
conveniently defined in C++ as \cppLstinline{Dt::Geom_traits}, where
\cppLstinline{Dt} is the triangulation instance. This type is exposed
as a Python attribute with the same name under
\pyLstinline{Triangulation_3} (which in turn is nested under the
Python namespace \pyLstinline{Tri3}).
Figure~\ref{fig:tri3:concept-hierarchy} depicts the 3D triangulation
traits concept hierarchy. Any kernel instance is a model of any
non-periodic traits concept; thus, when one of the templates
\begin{compactenum}
\item \cppLstinline{Triangulation_3<Traits, Tds>},
\item \cppLstinline{Regular_triangulation_3<Traits, Tds>}, abd
\item \cppLstinline{Delaunay_triangulation_3<Traits, Tds>}
\end{compactenum}
is instantiated, the \cppLstinline{Traits} parameter is substituted
with the \cppLstinline{Kernel} type (the selected kernel; see
Section~\ref{ssec:modules:kernel}). When one of the templates
\begin{compactenum}
\item \cppLstinline{Periodic_3_triangulation_3<Traits, Tds>},
\item \cppLstinline{Periodic_3_regular_triangulation_3<Traits, Tds>}, or
\item \cppLstinline{Periodic_3_Delaunay_triangulation_3<Traits, Tds>}
\end{compactenum}
is instantiated, the \cppLstinline{Traits} parameter is substituted
with \cppLstinline{Periodic_3_triangulation_traits_3<Kernel>},
\cppLstinline{Periodic_3_regular_triangulation_traits_3<Kernel>}, or
\cppLstinline{Periodic_3_Delaunay_triangulation_ traits_3<Kernel>},
respectively.
%
Observe that when a Delaunay triangulation instance is used to define
either a plain or a fixed alpha shape type (see
Section~\ref{ssec:modules:as3}), the traits parameter must be
substituted with a traits class that models either the
\cppLstinline{AlphaShapeTraits_3} or the
\cppLstinline{FixedAlphaShapeTraits_3} concept,
respectively. Similarly, when a regular triangulation instance is used
to define either a plain or a fixed alpha shape type (see
Section~\ref{ssec:modules:as3}, the traits parameter must be
substituted with a traits class that models either the
\cppLstinline{WeightedAlphaShapeTraits_3} or the
\cppLstinline{FixedWeightedAlphaShapeTraits_3} concept,
respectively. Also in these cases the selected kernel serves as the
traits.

\begin{figure}[!htp]
  \def\name#1{\scriptsize\cppLstinline{#1}}
  \tikzset{%
    concept/.style={rectangle,rounded corners,align=center,
      draw,fill=white,blur shadow,% drop shadow%
    }
  }
  \forestset{
    my tree style/.style={
      for tree={concept,
        parent anchor=south,
        child anchor=north,
        edge={->,>=stealth,black,thick},
        edge path={% |-| style branches from parent to child
          \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor)--(.child anchor)\forestoption{edge label};
        },
        if n children=3{% if a node has 3 children
          for children={% align the middle child with its parent
            if n=2{calign with current}{}
          }
        }{},
      }
    }
  }
  \centering
  \begin{forest}
    my tree style
    [ \name{TriTr3}
      [ \name{RegularTriTr3},name=r
        [ \name{WeightedASTr3} ]
        [ \name{FixedWeightedASTr3} ]
      ]
      [ \name{Periodic_3TriTr3},name=p
        [ \name{Pr3RegularTriTr3},name=pr ]
      ]
      [ \name{DelaunayTriTr3},name=d
        [ \name{Pr3DelaunayTriTr3},name=pd
	  [ \name{Pr3ASTr3} ]
        ]
        [ \name{ASTr3} ]
        [ \name{FixedASTr3} ]
      ]
    ]
    \draw[->,>=stealth] (r.parent anchor)--(pr.child anchor);
    \draw[->,>=stealth] (p.parent anchor)--(pd.child anchor);
  \end{forest}
  \caption{The 3D triangulation traits concept hierarchy.
    \cppLstinline{Triangulation}, \cppLstinline{AlphaShape},
    \cppLstinline{Traits_3} and \cppLstinline{Periodic_3} are
    abbreviated as \cppLstinline{Tri}, \cppLstinline{AS},
    \cppLstinline{Pr3}, and \cppLstinline{Tr3}, respectively.}
  \label{fig:tri3:concept-hierarchy}
\end{figure}

The \cmake{} Boolean flag \cmakeLstinline{CGALPY_TRI3_HIERARCHY} indicates
whether the type of triangulation, bindings for which should be
generated, is an instance of one of the triangulation hierarchy
templates, namely,
\begin{compactitem}
\item \cppLstinline{Triangulation_hierarchy_3<Triangulation_2>} and
\item \cppLstinline{Periodic_triangulation_hierarchy_3<PeriodicTriangulation_3>}.
\end{compactitem}
The template parameter in both cases is substituted with the
triangulation selected via the \cmake{} flag
\cmakeLstinline{CGALPY_TRI3_ NAME}, which also determines whether to use the
non-periodic or periodic version above.

The type that substitutes the \cppLstinline{Tds} parameter models the
concept \cppLstinline{TriangulationDataStructure_3}. An object of this
type stores the combinatorial structure of the triangulation; it is an
instance of the class template
\cppLstinline{Triangulation_data_structure_3<V, C, ConcurrencyTag>}.
The types that substitute the \cppLstinline{V} and \cppLstinline{C}
template parameters when the
\cppLstinline{Triangulation_data_structure_3<V, C>} template
is instantiated represent the type of the vertex and the type of the
cell of the triangulation, respectively; they must model the
\cppLstinline{TriangulationDS VertexBase_3} and
\cppLstinline{TriangulationDSCellBase_3} concepts, respectively. If the
binding is generated for a periodic triangulation, these parameters
must be substituted with types that also model the concepts
\cppLstinline{Periodic_3 TriangulationDSVertexBase_3} and
\cppLstinline{Periodic_3TriangulationDSCellBase_3}, respectively.
If the triangulation is used to define a plain alpha shape type, these
parameters must be substituted with types that model the concepts
\cppLstinline{AlphaShapeVertex_3} and
\cppLstinline{AlphaShapeCell_3}, respectively; see
Section~\ref{ssec:modules:as3}. If the triangulation is used to define
a fixed alpha shape type, these parameters must be substituted with
types that model the concepts \cppLstinline{FixedAlphaShapeVertex_3}
and \cppLstinline{FixedAlphaShapeCell_3}, respectively. Finally, if
the binding is generated for a hierarchy triangulation, e.g., an
instance of the template parameter
\cppLstinline{Triangulation_hierarchy_3<Triangulation_3>}, the
\cppLstinline{V} template parameter must be substituted with a model
of the concept \cppLstinline{Triangulation HierarchyVertexBase_3}.
(Observe that there is no special requirements on the type that
substitutes the \cppLstinline{C} parameter in this case.)
Similar to the 2D arrangement and 2D triangulation data structures,
it is possible to extend the vertex and cell types of the
triangulation. This is governed by two \cmake{} Boolean flags as
follows. If any one of the \cmake{} variables
\cmakeLstinline{CGALPY_TRI3_VERTEX_WITH_INFO} or
\cmakeLstinline{CGALPY_TRI3_CELL_WITH_INFO} is set to true, the
corresponding template parameter, \cppLstinline{V} or \cppLstinline{C},
is substituted with instances of
\cppLstinline{CGAL::Triangulation_vertex_base_ with_info_3<py::object, Traits, Vb>}
or
\cppLstinline{CGAL::Triangulation_cell_base_with_info_3<py::object, Traits, Cb>},
respectively, where
\cppLstinline{Vb} and \cppLstinline{Cb} are types that model the
concepts above. The final vertex type is selected accordingly; it is
explained in details in Section~\ref{sec:extenders:iiitri} of the appendix.

The final vertex type is conveniently defined in C++ as
\cppLstinline{Dt::Vertex}, where \cppLstinline{Dt} is the
triangulation instance. This type is exposed as a Python attribute
with the same name under \pyLstinline{Triangulation_3}.
%
The final face type is conveniently defined in C++ as
\cppLstinline{Dt::Face}, where \cppLstinline{Dt} is the triangulation
instance. This type is also exposed as a Python attribute with the
same name under \pyLstinline{Triangulation_3}.

The template parameter \cppLstinline{ConcurrencyTag} is substituted
with either \cppLstinline{Sequential_tag} or
\cppLstinline{Parallel_tag} when the template
\cppLstinline{Triangulation_data_structure_3<V, C, ConcurrencyTag} is
instantiated. It enables the use of a concurrent
container to store vertices and cells. The \cmake{} flag
\cmakeLstinline{CGALPY_TRI3_CONCURRENCY_NAME} determines the selection; see
Table~\ref{tab:tri3:concurrency}.

\begin{table}[!htp]
  \caption{3D triangulation concurrency options}
  \centering\begin{tikzpicture}
  \matrix (first) [tableName,
    column 1/.style={nodes={text width=18em}},
    column 2/.style={nodes={text width=31em}}
  ] {
    \cmakeLstinline{TRI3_CONCURRENCY_NAME} & Type\\
    \myLstinline{sequential} & \cppLstinline{Sequential_tag}\\
    \myLstinline{parallel} & \cppLstinline{Parallel_tag}\\
  };
  \end{tikzpicture}
  \label{tab:tri3:concurrency}
\end{table}

The template parameter \cppLstinline{LocationPolicy} is substituted
with either \cppLstinline{Fast_location} or
\cppLstinline{Compact_location} when the template
\cppLstinline{Delaunay_triangulation_3<Traits, Tds, LocationPolicy>}
is instantiated. It enables a faster point location at the account of
memory space. This is useful when performing point locations or random
point insertions in large data sets.  The \cmake{} flag
\cmakeLstinline{CGALPY_TRI3_LOCATION_POLICY_NAME} determines the
selection; see Table~\ref{tab:tri3:location}.

\begin{table}[!htp]
  \caption{3D triangulation location policy options}
  \centering\begin{tikzpicture} \matrix (first) [tableName, column
    1/.style={nodes={text width=18em}}, column 2/.style={nodes={text
        width=31em}} ] {
    \cmakeLstinline{TRI3_LOCATION_POLICY_NAME} & Type\\ \myLstinline{fast} &
    \cppLstinline{Fast_location}\\ \myLstinline{compact} &
    \cppLstinline{Compact_location}\\ };
  \end{tikzpicture}
  \label{tab:tri3:location}
\end{table}

The code excerpt in the \cmake{} language shown in
Listing~\ref{lst:cmake:tri2} sets the \cmake{} flags for our next
example in Python shown in Listing~\ref{lst:py:tri3}. The example
constructs a three-dimensional Delaunay triangulation from six points
and verifies that the triangulation is valid.

\begin{lstfloat}
  \def\filename{tri3_del_epic_release.cmake}%
  \lstinputlisting[style=cmakeFramedStyle,basicstyle=\normalsize,
                   label={lst:cmake:tri2},
                   caption={\cmake{} flag settings used to generate bindings for 3D triangulations.}]
                  {\cmakeDir\filename}
\end{lstfloat}

\begin{lstfloat}
  \def\filename{tri3_del.py}%
  \lstinputlisting[style=pythonFramedStyle,basicstyle=\normalsize,
                   firstline=15,
                   label={lst:py:tri3},
                   caption={Constructing a 3D~triangulations of six vertices.}]
                  {\pythonDir\filename}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsection{3D Alpha Shape Bindings}
\label{ssec:modules:as3}
% -----------------------------------------------------------------------------
Given a set of points sampled in a 3D body, an alpha shape
(a.k.a.\ alpha complex) is demarcated by a frontier, which is a linear
approximation of the original boundary of the body. Similar to the 2D
alpha shape object, A 3D alpha shape object maintains an underlying 3D
triangulation of a set of input points. Basic alpha shapes are based
on the Delaunay triangulation and weighted alpha shapes are based on
regular triangulation, where the euclidean distance is replaced by the
power to weighted points. The package
\iiiDAlphaShapesPackage{}~\cite{cgal:dy-as3-22} provides the class
templates \cppLstinline{Alpha_shape_3<Dt, ExactAlphaComparisonTag>}
and \cppLstinline{Fixed_alpha_shape_3<Dt>}. Instances of both
templates can be used to represent a large variety of alpha shapes for
a given set of points. In a plain alpha shape each $k$-face of this
triangulation is associated with an interval specifying for which
values of $\alpha$ the face belongs to the alpha complex. In a fixed
alpha shape each $k$-face is associated with a classification that
specifies its status in the alpha complex, alpha being
fixed. Table~\ref{tab:as3} lists the \cmake{} flags associated with
the \iiiDAlphaShapesPackage{} module.

%%%%%%%% 3D Alpha Shape flags
\begin{table}[!htp]
  \caption{\iiiDAlphaShapesPackage{} module flags}
  \centering\begin{tikzpicture}
  \matrix (first) [tableModuleFlags,
    column 1/.style={nodes={text width=16em}},
    column 3/.style={nodes={text width=5.7em}},
    column 4/.style={nodes={text width=21.6em}}
  ] {
Name & Type &  Default & Description\\
\myLstinline{AS3_NAME}              & String  & \myLstinline{plain} & The 3D Alpha shape type\\
\myLstinline{AS3_EXACT_COMPARISON} & Boolean & \myLstinline{false} & Determines whether to apply exact comparisons\\
  };
 \end{tikzpicture}
 \label{tab:as3}
\end{table}

The \cmake{} flag \myLstinline{AS3_NAME} specifies which alpha shape
should be used for the generated bindings; see
Table~\ref{tab:as3:types}

%%%%%%%% 3D Alpha Shapes Module Types
\begin{table}[!htp]
 \caption{\iiiDAlphaShapesPackage{} types}
  \centering\begin{tikzpicture}
  \matrix (first) [tableName,
    column 1/.style={nodes={text width=12em}},
    column 2/.style={nodes={text width=37em}}
  ] {
     \myLstinline{AS3_NAME} & Type\\
     \myLstinline{plain} & \cppLstinline{Alpha_shape_3<Tri, Ec>}\\
     \myLstinline{fixed} & \cppLstinline{Fixed_alpha_shape_3<Tri>}\\
  };
 \end{tikzpicture}
 \label{tab:as3:types}
\end{table}

The template parameter \cppLstinline{Dt} must be substituted with an
instance of one of the following class templates that can be used to
represent a triangulation:
\begin{compactenum}
\item \cppLstinline{Delaunay_triangulation_3},
\item \cppLstinline{Regular_triangulation_3},
\item \cppLstinline{Periodic_3_Delaunay_triangulation_3}, or
\item \cppLstinline{Periodic_3_regular_triangulation_3};
\end{compactenum}
see Section~\ref{ssec:modules:tri3}.  Note that
\cppLstinline{Dt::Geom_traits} must be model of a suitable alpha-shape
traits concept, and \cppLstinline{Dt::Vertex} and
\cppLstinline{Dt::Face} must be models suitable alpha-shape vertex and
cell concepts, respectively; see Section~\ref{ssec:modules:tri3}.

The following code excerpt in the \cmake{} language shown in
Listing~\ref{lst:cmake:as3} sets the \cmake{} flags for our next
Python example shown in Listing~\ref{lst:py:as3}. The examples
constructs an alpha shape object.

\begin{lstfloat}
  \def\filename{as3_del_compact_parallel_epic_release.cmake}%
  \lstinputlisting[style=cmakeFramedStyle,basicstyle=\normalsize,
                   label={lst:cmake:as3},
                   caption={\cmake{} flag settings used to generate bindings for 3D alpha shapes.}]
                  {\cmakeDir\filename}
\end{lstfloat}

\begin{lstfloat}
  \def\filename{as3_del_compact_epic.py}%
  \lstinputlisting[style=pythonFramedStyle,basicstyle=\normalsize,
                   firstline=15,
                   label={lst:py:as3},
                   caption={Constructing a 3D alpha shape object.}]
                  {\pythonDir\filename}
\end{lstfloat}

% -----------------------------------------------------------------------------
\subsection{Spatial Searching Bindings}
\label{ssec:modules:ss}
% -----------------------------------------------------------------------------
The \dDSpatialSearchingPackage{} package~\cite{cgal:tf-ssd-22}
implements exact and approximate distance browsing by providing
implementations of algorithms supporting
\begin{compactenum}
\item both nearest and furthest neighbor searching,
\item both exact and approximate searching,
\item (approximate) range searching,
\item (approximate) $k$-nearest and $k$-furthest neighbor searching,
\item (approximate) incremental nearest and incremental furthest neighbor searching, and
\item query items representing points and spatial objects.
\end{compactenum}
In these searching problems a set $\calP$ of data points in
$d$-dimensional space is given. The points in $\calP$ are preprocessed
into a tree data structure, so that given any query item $q$ the
points of $\calP$ can be browsed efficiently. The approximate
\dDSpatialSearchingPackage{} package is designed for data sets that
are small enough to store the search structure in main memory (in
contrast to approaches from databases that assume that the data reside
in secondary storage).

%%%%%%%%
\begin{table}[!htp]
  \caption{\dDSpatialSearchingPackage{} module flags}
  \centering\begin{tikzpicture}
  \matrix (first) [tableModuleFlags,
    column 3/.style={nodes={text width=3.5em}},
    column 4/.style={nodes={text width=21.8em}}
  ] {
    Name & Type &  Default & Description\\
    \cmakeLstinline{SPATIAL_SEARCHING_DIMENSION} & Integer & \cppLstinline{2} &
      The dimension of spatial searching related classes\\
  };
 \end{tikzpicture}
 \label{tab:ss}
\end{table}

The code excerpt in the \cmake{} language shown in
Listing~\ref{lst:cmake:ss}, sets the \cmake{} flags for our last
example shown in Listing~\ref{lst:py:ss}. The example constructs a
\kdtree{} of 2D points and applies various queries on the tree.
Observe that the \kdtree{} dimension (and the dimension of related
data structures) is set via the \cmake{} flag
\myLstinline{CGALPY_SPATIAL_SEARCHING_DIMENSION} during compile time.
The code in the listings assumes that the dimension is~2. In order to
assert the dimension the bindings were compiled with (see Line~10 in
the listing), we have introduced and exposed a free function called
\myLstinline{get_spatial_searching_dimension()} that returns the
dimension as an \pyLstinline{int}.

\begin{lstfloat}
  \def\filename{ss_2_cdlg_release.cmake}%
  \lstinputlisting[style=cmakeFramedStyle,basicstyle=\normalsize,
                   label={lst:cmake:ss},
                   caption={\cmake{} flag settings used to generate bindings for spatial searching types.}]
                  {\cmakeDir\filename}
\end{lstfloat}

\begin{lstfloat}
  \def\filename{kd_tree.py}
  \lstinputlisting[style=pythonFramedStyle,basicstyle=\normalsize,
                   label={lst:py:ss},
                   firstline=17,
                   lastline=64,
                   caption={Applying various queries on a \kdtree{} of 2D points.}]
                  {\pythonDir\filename}
\end{lstfloat}

%% 2. kernel-d is used by spatial searching

